Predicted Yield of Transits of Known Radial Velocity Exoplanets from the TESS Primary and Extended Missions

Radial velocity (RV) surveys have detected hundreds of exoplanets through their gravitational interactions with their host stars. Some will be transiting, but most lack sufficient follow-up observations to confidently detect (or rule out) transits. We use published stellar, orbital, and planetary parameters to estimate the transit probabilities for nearly all exoplanets that have been discovered via the RV method. From these probabilities, we predict that $25.5^{+0.7}_{-0.7}$ of the known RV exoplanets should transit their host stars. This prediction is more than double the amount of RV exoplanets that are currently known to transit. The Transiting Exoplanet Survey Satellite (TESS) presents a valuable opportunity to explore the transiting nature of many of the known RV exoplanet systems. Based on the anticipated pointing of TESS during its two-year primary mission, we identify the known RV exoplanets that it will observe and predict that $11.7^{+0.3}_{-0.3}$ of them will have transits detected by TESS. However, we only expect the discovery of transits for $\sim$3 of these exoplanets to be novel (i.e., not previously known). We predict that the TESS photometry will yield dispositive null results for the transits of $\sim$125 RV exoplanets. This will represent a substantial increase in the effort to refine ephemerides of known RV exoplanets. We demonstrate that these results are robust to changes in the ecliptic longitudes of future TESS observing sectors. Finally, we consider how several potential TESS extended mission scenarios affect the number of transiting RV exoplanets we expect TESS to observe.

==> all_planets_table.tex <==
NGC 2682 Sand 364 b & 294684871 & 0.5$^{+0.5}_{-0.5}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
BD+20 2457 b & 99734092 & 0.4$^{+0.4}_{-0.4}$ & 0.03$^{+0.03}_{-0.03}$ & \nodata & \nodata & 8 & 1\\
55 Cnc e & 332064670 & 0.291$^{+0.005}_{-0.004}$ & 0.291$^{+0.005}_{-0.004}$ & \nodata & \nodata & 7 & 1\\
HD 240237 b & 323919676 & 0.29$^{+0.1}_{-0.08}$ & 0.021$^{+0.007}_{-0.006}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 102956 b & 428673146 & 0.28$^{+0.03}_{-0.03}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 86081 b & 27073220 & 0.27$^{+0.03}_{-0.03}$ & 0.27$^{+0.03}_{-0.03}$ & 8 & 1 & \nodata & \nodata\\
24 Boo b & 441712711 & 0.26$^{+0.03}_{-0.02}$ & 0.26$^{+0.03}_{-0.02}$ & \nodata & \nodata & 9,10 & 3,3\\
HD 96127 b & 268634769 & 0.2$^{+0.1}_{-0.1}$ & 0.01$^{+0.005}_{-0.005}$ & \nodata & \nodata & 8 & 2\\
HD 88133 b & 54237857 & 0.23$^{+0.03}_{-0.03}$ & 0.23$^{+0.03}_{-0.03}$ & \nodata & \nodata & 8 & 1\\
HD 24064 b & 286923464 & 0.22$^{+0.04}_{-0.03}$ & 0.022$^{+0.004}_{-0.003}$ & \nodata & \nodata & 5,6 & 2,2\\
HD 118203 b & 120960812 & 0.21$^{+0.02}_{-0.02}$ & 0.21$^{+0.02}_{-0.02}$ & \nodata & \nodata & 9 & 3\\
GJ 674 b & 20096620 & 0.2$^{+0.2}_{-0.2}$ & 0.2$^{+0.2}_{-0.2}$ & 12 & 1 & \nodata & \nodata\\
HD 1690 b & 37763102 & 0.21$^{+0.07}_{-0.06}$ & 0.01$^{+0.003}_{-0.003}$ & 3 & 1 & \nodata & \nodata\\
WASP-94 B b & 68418284 & 0.21$^{+0.02}_{-0.02}$ & 0.21$^{+0.02}_{-0.02}$ & 1 & 1 & \nodata & \nodata\\
HD 212301 b & 161314759 & 0.2$^{+0.02}_{-0.02}$ & 0.2$^{+0.02}_{-0.02}$ & 1,13 & 3,3 & \nodata & \nodata\\
HD 13189 b & 63564248 & 0.2$^{+0.03}_{-0.03}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
BD+20 2457 c & 148563075 & 0.2$^{+0.2}_{-0.2}$ & 0.008$^{+0.009}_{-0.008}$ & \nodata & \nodata & 8 & 1\\
HD 143105 b & 316470945 & 0.19$^{+0.01}_{-0.01}$ & 0.19$^{+0.01}_{-0.01}$ & \nodata & \nodata & 1,2,3,4,6,7,8,9,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4\\
HD 220074 b & 269237357 & 0.19$^{+0.04}_{-0.03}$ & 0.015$^{+0.003}_{-0.003}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 185269 b & 213721036 & 0.18$^{+0.02}_{-0.02}$ & 0.18$^{+0.02}_{-0.02}$ & \nodata & \nodata & 1 & 2\\
V830 Tau b & 406320735 & 0.17$^{+0.02}_{-0.02}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 95127 b & 82308728 & 0.17$^{+0.08}_{-0.08}$ & 0.009$^{+0.005}_{-0.004}$ & \nodata & \nodata & 8 & 2\\
HD 149143 b & 124165580 & 0.17$^{+0.02}_{-0.02}$ & 0.17$^{+0.02}_{-0.02}$ & \nodata & \nodata & 12 & 1\\
HD 80606 b & 446137194 & 0.16$^{+0.02}_{-0.01}$ & 0.039$^{+0.004}_{-0.003}$ & \nodata & \nodata & 7 & 2\\
HD 149026 b & 353181458 & 0.16$^{+0.02}_{-0.01}$ & 0.16$^{+0.02}_{-0.01}$ & \nodata & \nodata & 11,12 & 3,3\\
HD 179949 b & 410399074 & 0.16$^{+0.08}_{-0.08}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
tau Boo b & 72506701 & 0.15$^{+0.01}_{-0.01}$ & 0.15$^{+0.01}_{-0.01}$ & \nodata & \nodata & 10 & 1\\
HD 76700 b & 457134360 & 0.15$^{+0.02}_{-0.02}$ & 0.15$^{+0.02}_{-0.02}$ & 5,9,10,11 & 4,3,3,3 & \nodata & \nodata\\
GJ 3138 b & 471012347 & 0.15$^{+0.04}_{-0.02}$ & 0.15$^{+0.04}_{-0.02}$ & 3 & 1 & \nodata & \nodata\\
HD 219828 b & 114807081 & 0.15$^{+0.02}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 17156 b & 302773669 & 0.144$^{+0.006}_{-0.006}$ & 0.144$^{+0.006}_{-0.006}$ & \nodata & \nodata & 5 & 2\\
TYC 4282-00605-1 b & 115869504 & 0.14$^{+0.04}_{-0.04}$ & 0.08$^{+0.02}_{-0.02}$ & \nodata & \nodata & 3,4 & 3,3\\
4 UMa b & 414965996 & 0.14$^{+0.01}_{-0.01}$ & 0.014$^{+0.001}_{-0.001}$ & \nodata & \nodata & 7 & 2\\
HD 125612 c & 349606708 & 0.14$^{+0.03}_{-0.02}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
Pr0211 b & 270730826 & 0.139$^{+0.004}_{-0.004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 20782 b & 144503325 & 0.14$^{+0.07}_{-0.03}$ & 0.006$^{+0.003}_{-0.002}$ & 4 & 2 & \nodata & \nodata\\
bet Cnc b & 471011652 & 0.139$^{+0.01}_{-0.009}$ & 0.0062$^{+0.0004}_{-0.0004}$ & 7 & 1 & \nodata & \nodata\\
TYC 3667-1280-1 b & 225317852 & 0.14$^{+0.02}_{-0.02}$ & 0.14$^{+0.02}_{-0.02}$ & \nodata & \nodata & 4 & 2\\
HD 46375 b & 234928947 & 0.13$^{+0.07}_{-0.07}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
alf Tau b & 95361265 & 0.13$^{+0.03}_{-0.02}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 189733 b & 256364928 & 0.13$^{+0.01}_{-0.01}$ & 0.13$^{+0.01}_{-0.01}$ & \nodata & \nodata & 1 & 2\\
ups And b & 382073690 & 0.13$^{+0.06}_{-0.06}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 75289 b & 468723402 & 0.13$^{+0.02}_{-0.01}$ & 0.13$^{+0.02}_{-0.01}$ & 8,9 & 3,3 & \nodata & \nodata\\
HD 73256 b & 181741837 & 0.13$^{+0.01}_{-0.01}$ & 0.13$^{+0.01}_{-0.01}$ & 8 & 2 & \nodata & \nodata\\
HD 209458 b & 420814525 & 0.126$^{+0.01}_{-0.009}$ & 0.126$^{+0.01}_{-0.009}$ & \nodata & \nodata & 2 & 1\\
HD 83443 b & 22221375 & 0.12$^{+0.01}_{-0.01}$ & 0.12$^{+0.01}_{-0.01}$ & 9 & 2 & \nodata & \nodata\\
HD 2638 b & 244178536 & 0.12$^{+0.01}_{-0.01}$ & 0.12$^{+0.01}_{-0.01}$ & 3 & 1 & \nodata & \nodata\\
HD 216536 b & 156067565 & 0.12$^{+0.04}_{-0.03}$ & 0.022$^{+0.006}_{-0.005}$ & \nodata & \nodata & 3 & 2\\
BD-10 3166 b & 247119634 & 0.12$^{+0.02}_{-0.01}$ & 0.12$^{+0.02}_{-0.01}$ & 9 & 1 & \nodata & \nodata\\
HIP 63242 b & 437310271 & 0.12$^{+0.03}_{-0.03}$ & 0.026$^{+0.007}_{-0.006}$ & 11 & 2 & \nodata & \nodata\\
HD 187123 b & 58559140 & 0.12$^{+0.009}_{-0.008}$ & 0.12$^{+0.009}_{-0.008}$ & \nodata & \nodata & 1 & 3\\
gam 1 Leo b & 9815387 & 0.12$^{+0.007}_{-0.007}$ & 0.0075$^{+0.0004}_{-0.0004}$ & \nodata & \nodata & 8 & 1\\
51 Peg b & 444865362 & 0.12$^{+0.05}_{-0.05}$ & 0.12$^{+0.05}_{-0.05}$ & \nodata & \nodata & 2 & 1\\
NGC 2682 YBP 401 b & 437030651 & 0.118$^{+0.009}_{-0.009}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 158996 b & 288268410 & 0.12$^{+0.02}_{-0.01}$ & 0.027$^{+0.004}_{-0.003}$ & \nodata & \nodata & 1,4,5,6,7,8,11 & 4,4,4,3,3,4,4\\
BD+48 740 b & 71099944 & 0.11$^{+0.04}_{-0.03}$ & 0.004$^{+0.001}_{-0.001}$ & \nodata & \nodata & 5 & 2\\
HIP 75458 b & 32448045 & 0.11$^{+0.03}_{-0.03}$ & 0.018$^{+0.006}_{-0.005}$ & \nodata & \nodata & 8,9,10 & 3,3,3\\
HD 330075 b & 275786473 & 0.11$^{+0.01}_{-0.01}$ & 0.11$^{+0.01}_{-0.01}$ & 12 & 1 & \nodata & \nodata\\
bet UMi b & 229540730 & 0.113$^{+0.009}_{-0.008}$ & 0.023$^{+0.002}_{-0.002}$ & \nodata & \nodata & 6,7,8,9 & 3,3,3,3\\
HD 33283 b & 66650754 & 0.11$^{+0.02}_{-0.01}$ & 0.11$^{+0.02}_{-0.01}$ & 5 & 2 & \nodata & \nodata\\
BD+15 2940 b & 158917706 & 0.11$^{+0.03}_{-0.02}$ & 0.022$^{+0.006}_{-0.005}$ & \nodata & \nodata & 11 & 2\\
tau Gem b & 375464367 & 0.11$^{+0.01}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 47186 b & 101145648 & 0.11$^{+0.01}_{-0.01}$ & 0.11$^{+0.01}_{-0.01}$ & 6,7 & 2,2 & \nodata & \nodata\\
HD 11755 b & 257005016 & 0.11$^{+0.02}_{-0.02}$ & 0.007$^{+0.001}_{-0.001}$ & \nodata & \nodata & 5 & 3\\
HD 109749 b & 422214062 & 0.11$^{+0.01}_{-0.01}$ & 0.11$^{+0.01}_{-0.01}$ & 10 & 2 & \nodata & \nodata\\
BD+03 2562 b & 419015728 & 0.11$^{+0.03}_{-0.03}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 208527 b & 356473029 & 0.11$^{+0.02}_{-0.02}$ & 0.0033$^{+0.0007}_{-0.0006}$ & \nodata & \nodata & 2 & 2\\
8 UMi b & 255480497 & 0.11$^{+0.01}_{-0.01}$ & 0.11$^{+0.01}_{-0.01}$ & \nodata & \nodata & 6,7,8,9 & 3,3,3,3\\
HD 76920 b & 302070274 & 0.1$^{+0.01}_{-0.01}$ & 0.02$^{+0.002}_{-0.002}$ & 9,10,11 & 3,3,3 & \nodata & \nodata\\
NGC 2682 YBP 1194 b & 175291727 & 0.1$^{+0.01}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 63454 b & 165796397 & 0.1$^{+0.01}_{-0.01}$ & 0.1$^{+0.01}_{-0.01}$ & 3,4,7,10,11,12,13 & 4,4,4,4,3,3,4 & \nodata & \nodata\\
HD 113996 b & 437039060 & 0.1$^{+0.02}_{-0.02}$ & 0.0045$^{+0.001}_{-0.0007}$ & \nodata & \nodata & 9 & 2\\
HD 103774 b & 66666079 & 0.1$^{+0.02}_{-0.02}$ & 0.1$^{+0.02}_{-0.02}$ & 9 & 1 & \nodata & \nodata\\
HD 12648 b & 101555167 & 0.1$^{+0.01}_{-0.009}$ & 0.04$^{+0.004}_{-0.004}$ & \nodata & \nodata & 5,6 & 3,3\\
HD 102272 b & 400806831 & 0.1$^{+0.01}_{-0.01}$ & 0.021$^{+0.003}_{-0.002}$ & \nodata & \nodata & 9 & 1\\
HD 68988 b & 165796397 & 0.099$^{+0.01}_{-0.009}$ & 0.099$^{+0.01}_{-0.009}$ & \nodata & \nodata & 7 & 2\\
Pr0201 b & 450417907 & 0.1$^{+0.01}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
11 UMi b & 72437047 & 0.1$^{+0.01}_{-0.01}$ & 0.031$^{+0.004}_{-0.003}$ & \nodata & \nodata & 3,6,7,8,9,13 & 4,4,3,3,3,4\\
61 Vir b & 332064670 & 0.098$^{+0.01}_{-0.008}$ & 0.098$^{+0.01}_{-0.008}$ & 10 & 1 & \nodata & \nodata\\
HD 1461 b & 246835467 & 0.098$^{+0.007}_{-0.007}$ & 0.098$^{+0.007}_{-0.007}$ & 3 & 1 & \nodata & \nodata\\
HD 215497 b & 38271828 & 0.1$^{+0.02}_{-0.01}$ & 0.1$^{+0.02}_{-0.01}$ & 1 & 2 & \nodata & \nodata\\
HD 219134 b & 175291727 & 0.096$^{+0.002}_{-0.002}$ & 0.096$^{+0.002}_{-0.002}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 49674 b & 344627954 & 0.09$^{+0.01}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 69830 b & 11665403 & 0.09$^{+0.09}_{-0.09}$ & 0.09$^{+0.09}_{-0.09}$ & 7 & 2 & \nodata & \nodata\\
HD 168746 b & 228217280 & 0.09$^{+0.01}_{-0.01}$ & 0.09$^{+0.01}_{-0.01}$ & \nodata & \nodata & 13 & 1\\
11 Com b & 48237215 & 0.09$^{+0.01}_{-0.01}$ & 0.0074$^{+0.0008}_{-0.0008}$ & \nodata & \nodata & 9 & 1\\
HIP 14810 b & 111947706 & 0.089$^{+0.01}_{-0.009}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 102195 b & 137810576 & 0.088$^{+0.01}_{-0.008}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 40307 b & 374859347 & 0.09$^{+0.02}_{-0.02}$ & 0.09$^{+0.02}_{-0.02}$ & 1,2,3,4,5,6,7,8,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4 & \nodata & \nodata\\
HD 77338 b & 302580456 & 0.09$^{+0.03}_{-0.02}$ & 0.09$^{+0.03}_{-0.02}$ & 8 & 2 & \nodata & \nodata\\
CoRoT-7 c & 440955228 & 0.087$^{+0.01}_{-0.009}$ & 0.087$^{+0.01}_{-0.009}$ & 6 & 1 & \nodata & \nodata\\
HD 66141 b & 382625142 & 0.086$^{+0.008}_{-0.007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 5891 b & 243146568 & 0.084$^{+0.01}_{-0.009}$ & 0.013$^{+0.002}_{-0.001}$ & \nodata & \nodata & 3 & 1\\
HD 163607 b & 353988778 & 0.083$^{+0.008}_{-0.007}$ & 0.083$^{+0.008}_{-0.007}$ & \nodata & \nodata & 1,2,3,4,5,6,7,8,9,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4,4\\
xi Aql b & 283722336 & 0.08$^{+0.04}_{-0.04}$ & 0.016$^{+0.008}_{-0.008}$ & \nodata & \nodata & 1 & 1\\
HD 3167 d & 318707987 & 0.083$^{+0.004}_{-0.004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 217107 b & 243085377 & 0.082$^{+0.009}_{-0.008}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 38529 b & 200093173 & 0.08$^{+0.08}_{-0.08}$ & 0.08$^{+0.08}_{-0.08}$ & 6 & 1 & \nodata & \nodata\\
eps CrB b & 82204610 & 0.08$^{+0.04}_{-0.04}$ & 0.005$^{+0.003}_{-0.003}$ & \nodata & \nodata & 11 & 2\\
HD 32518 b & 310836777 & 0.082$^{+0.008}_{-0.008}$ & 0.028$^{+0.003}_{-0.003}$ & \nodata & \nodata & 5,6 & 2,2\\
GJ 436 b & 57654763 & 0.081$^{+0.006}_{-0.006}$ & 0.081$^{+0.006}_{-0.006}$ & \nodata & \nodata & 9 & 1\\
GJ 3998 b & 388857263 & 0.081$^{+0.009}_{-0.008}$ & 0.081$^{+0.009}_{-0.008}$ & \nodata & \nodata & 12 & 2\\
HD 10180 c & 180205814 & 0.081$^{+0.004}_{-0.004}$ & 0.081$^{+0.004}_{-0.004}$ & 1,2 & 3,3 & \nodata & \nodata\\
HD 5583 b & 53848538 & 0.08$^{+0.02}_{-0.01}$ & 0.016$^{+0.003}_{-0.003}$ & \nodata & \nodata & 4 & 1\\
HIP 91258 b & 383675945 & 0.08$^{+0.009}_{-0.008}$ & 0.08$^{+0.009}_{-0.008}$ & \nodata & \nodata & 2,3,4,5,6,7,8,9,10,12,13 & 4,4,4,4,4,4,4,4,4,4,4\\
HD 181433 b & 134245358 & 0.08$^{+0.01}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 179079 b & 12192000 & 0.08$^{+0.01}_{-0.01}$ & 0.08$^{+0.01}_{-0.01}$ & \nodata & \nodata & 13 & 1\\
HIP 107773 b & 11782681 & 0.08$^{+0.01}_{-0.01}$ & 0.015$^{+0.002}_{-0.002}$ & 1 & 2 & \nodata & \nodata\\
42 Dra b & 1713457 & 0.077$^{+0.007}_{-0.006}$ & 0.048$^{+0.004}_{-0.004}$ & \nodata & \nodata & 1,3,4,5,6,7,8,9,10,11,13 & 4,4,4,4,4,4,4,4,4,4,4\\
GJ 3470 b & 218263393 & 0.077$^{+0.01}_{-0.009}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 3634 b & 124401411 & 0.077$^{+0.009}_{-0.008}$ & 0.077$^{+0.009}_{-0.008}$ & 9 & 2 & \nodata & \nodata\\
HD 100655 b & 306349516 & 0.077$^{+0.009}_{-0.009}$ & 0.013$^{+0.002}_{-0.001}$ & \nodata & \nodata & 9 & 1\\
BD+20 274 b & 37748347 & 0.08$^{+0.01}_{-0.01}$ & 0.0035$^{+0.0005}_{-0.0005}$ & \nodata & \nodata & 4 & 1\\
HD 81688 b & 8915600 & 0.08$^{+0.04}_{-0.04}$ & 0.011$^{+0.006}_{-0.005}$ & \nodata & \nodata & 7 & 1\\
BD+15 2375 b & 82604982 & 0.08$^{+0.02}_{-0.01}$ & 0.013$^{+0.003}_{-0.002}$ & \nodata & \nodata & 9 & 1\\
NGC 2682 Sand 978 b & 290172418 & 0.074$^{+0.01}_{-0.009}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
91 Aqr b & 118572803 & 0.074$^{+0.008}_{-0.007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 103720 b & 176910071 & 0.074$^{+0.003}_{-0.003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 145457 b & 350083732 & 0.073$^{+0.006}_{-0.006}$ & 0.0112$^{+0.0009}_{-0.0008}$ & \nodata & \nodata & 11 & 2\\
alf Ari b & 356000102 & 0.072$^{+0.009}_{-0.007}$ & 0.0051$^{+0.0006}_{-0.0005}$ & \nodata & \nodata & 4 & 1\\
NGC 2682 YBP 1514 b & 437034946 & 0.072$^{+0.008}_{-0.007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
omi CrB b & 357502856 & 0.07$^{+0.01}_{-0.01}$ & 0.01$^{+0.002}_{-0.001}$ & \nodata & \nodata & 11 & 2\\
GJ 676 A d & 248027247 & 0.07$^{+0.01}_{-0.01}$ & 0.07$^{+0.01}_{-0.01}$ & 12 & 1 & \nodata & \nodata\\
HD 162020 b & 159019691 & 0.07$^{+0.008}_{-0.007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 285507 b & 389018596 & 0.069$^{+0.008}_{-0.007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
NGC 4349 127 b & 115779095 & 0.07$^{+0.02}_{-0.02}$ & 0.0027$^{+0.001}_{-0.0009}$ & 11 & 2 & \nodata & \nodata\\
HD 156668 b & 348652846 & 0.069$^{+0.001}_{-0.001}$ & 0.069$^{+0.001}_{-0.001}$ & \nodata & \nodata & 12 & 2\\
BD-13 2130 b & 33355302 & 0.07$^{+0.02}_{-0.02}$ & 0.0026$^{+0.0008}_{-0.0007}$ & 7 & 2 & \nodata & \nodata\\
BD-08 2823 b & 230183006 & 0.07$^{+0.02}_{-0.01}$ & 0.07$^{+0.02}_{-0.01}$ & 8 & 1 & \nodata & \nodata\\
BD-06 1339 b & 60923874 & 0.067$^{+0.004}_{-0.004}$ & 0.067$^{+0.004}_{-0.004}$ & 6 & 1 & \nodata & \nodata\\
HD 7924 b & 468723402 & 0.066$^{+0.008}_{-0.007}$ & 0.066$^{+0.008}_{-0.007}$ & \nodata & \nodata & 5 & 3\\
HD 233604 b & 150184553 & 0.066$^{+0.009}_{-0.007}$ & 0.009$^{+0.001}_{-0.001}$ & \nodata & \nodata & 7 & 2\\
HIP 57274 b & 5078530 & 0.07$^{+0.01}_{-0.01}$ & 0.07$^{+0.01}_{-0.01}$ & \nodata & \nodata & 9 & 1\\
HD 16417 b & 53134037 & 0.07$^{+0.07}_{-0.06}$ & 0.07$^{+0.07}_{-0.06}$ & 3,4 & 2,2 & \nodata & \nodata\\
HD 1461 c & 305837711 & 0.066$^{+0.005}_{-0.004}$ & 0.066$^{+0.005}_{-0.004}$ & 3 & 1 & \nodata & \nodata\\
HD 87646 b & 27064335 & 0.064$^{+0.009}_{-0.009}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
K2-18 c & 301051051 & 0.064$^{+0.007}_{-0.007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 876 d & 178872239 & 0.06$^{+0.03}_{-0.03}$ & 0.06$^{+0.03}_{-0.03}$ & 2 & 1 & \nodata & \nodata\\
HD 109271 b & 30293512 & 0.063$^{+0.009}_{-0.008}$ & 0.063$^{+0.009}_{-0.008}$ & 10 & 1 & \nodata & \nodata\\
HIP 67851 b & 429301734 & 0.062$^{+0.006}_{-0.006}$ & 0.019$^{+0.002}_{-0.002}$ & 11 & 1 & \nodata & \nodata\\
14 And b & 230061010 & 0.062$^{+0.009}_{-0.008}$ & 0.009$^{+0.001}_{-0.001}$ & \nodata & \nodata & 3 & 2\\
TAP 26 b & 290172418 & 0.062$^{+0.009}_{-0.008}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 117618 b & 347909637 & 0.06$^{+0.03}_{-0.01}$ & 0.06$^{+0.03}_{-0.01}$ & 11 & 2 & \nodata & \nodata\\
HD 219134 c & 264508014 & 0.06$^{+0.003}_{-0.002}$ & 0.06$^{+0.003}_{-0.002}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 215152 b & 251042502 & 0.06$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 59686 A b & 440955228 & 0.059$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
tau Cet g & 419015728 & 0.06$^{+0.06}_{-0.06}$ & 0.06$^{+0.06}_{-0.06}$ & 3 & 1 & \nodata & \nodata\\
HD 17092 b & 102264230 & 0.059$^{+0.007}_{-0.007}$ & 0.0044$^{+0.0005}_{-0.0005}$ & \nodata & \nodata & 5 & 2\\
HD 176986 b & 39554091 & 0.058$^{+0.005}_{-0.004}$ & 0.058$^{+0.005}_{-0.004}$ & \nodata & \nodata & 13 & 1\\
ome Ser b & 189576919 & 0.057$^{+0.009}_{-0.007}$ & 0.0055$^{+0.0009}_{-0.0007}$ & \nodata & \nodata & 11 & 1\\
HD 156846 b & 248320609 & 0.056$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 37605 b & 144730053 & 0.056$^{+0.01}_{-0.009}$ & 0.027$^{+0.006}_{-0.004}$ & 6 & 1 & \nodata & \nodata\\
HD 160691 d & 232620788 & 0.055$^{+0.007}_{-0.006}$ & 0.055$^{+0.007}_{-0.006}$ & 12 & 1 & \nodata & \nodata\\
GJ 3942 b & 254147274 & 0.06$^{+0.01}_{-0.01}$ & 0.06$^{+0.01}_{-0.01}$ & \nodata & \nodata & 9,10,11 & 3,3,3\\
HD 13908 b & 342041655 & 0.054$^{+0.003}_{-0.003}$ & 0.054$^{+0.003}_{-0.003}$ & \nodata & \nodata & 5 & 2\\
BD+48 738 b & 267519701 & 0.054$^{+0.01}_{-0.008}$ & 0.0037$^{+0.0007}_{-0.0006}$ & \nodata & \nodata & 5 & 2\\
HD 195019 b & 210171104 & 0.054$^{+0.006}_{-0.005}$ & 0.054$^{+0.006}_{-0.005}$ & \nodata & \nodata & 1 & 2\\
YZ Cet b & 207492082 & 0.053$^{+0.008}_{-0.007}$ & 0.053$^{+0.008}_{-0.007}$ & 3 & 1 & \nodata & \nodata\\
HD 104985 b & 450491293 & 0.05$^{+0.03}_{-0.03}$ & 0.007$^{+0.004}_{-0.004}$ & \nodata & \nodata & 7 & 3\\
HD 159243 b & 362661163 & 0.052$^{+0.003}_{-0.003}$ & 0.052$^{+0.003}_{-0.003}$ & \nodata & \nodata & 12 & 1\\
HD 215152 c & 251042502 & 0.051$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 11964 c & 24978373 & 0.05$^{+0.02}_{-0.01}$ & 0.036$^{+0.01}_{-0.008}$ & 3 & 1 & \nodata & \nodata\\
HD 6434 b & 180871947 & 0.05$^{+0.006}_{-0.005}$ & 0.05$^{+0.006}_{-0.005}$ & 2,3 & 2,2 & \nodata & \nodata\\
GJ 581 e & 139754153 & 0.05$^{+0.02}_{-0.02}$ & 0.05$^{+0.02}_{-0.02}$ & \nodata & \nodata & 11 & 1\\
TYC 1422-614-1 b & 183532609 & 0.05$^{+0.01}_{-0.01}$ & 0.007$^{+0.001}_{-0.001}$ & \nodata & \nodata & 8 & 1\\
HD 130322 b & 284680749 & 0.049$^{+0.006}_{-0.005}$ & 0.049$^{+0.006}_{-0.005}$ & \nodata & \nodata & 11 & 1\\
HD 40307 c & 219152539 & 0.048$^{+0.01}_{-0.009}$ & 0.048$^{+0.01}_{-0.009}$ & 1,2,3,4,5,6,7,8,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4 & \nodata & \nodata\\
HIP 105854 b & 129649472 & 0.05$^{+0.01}_{-0.01}$ & 0.007$^{+0.002}_{-0.002}$ & 1 & 1 & \nodata & \nodata\\
XO-2 S b & 456826468 & 0.048$^{+0.006}_{-0.005}$ & 0.048$^{+0.006}_{-0.005}$ & \nodata & \nodata & 7 & 1\\
GJ 3138 c & 43605290 & 0.048$^{+0.007}_{-0.005}$ & 0.048$^{+0.007}_{-0.005}$ & 3 & 1 & \nodata & \nodata\\
HD 2952 b & 436700755 & 0.047$^{+0.006}_{-0.005}$ & 0.0041$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & 4 & 2\\
Wolf 1061 b & 413948621 & 0.047$^{+0.01}_{-0.007}$ & 0.047$^{+0.01}_{-0.007}$ & \nodata & \nodata & 12 & 1\\
HD 47536 b & 52172862 & 0.046$^{+0.01}_{-0.007}$ & 0.0035$^{+0.0008}_{-0.0006}$ & 6,7 & 3,3 & \nodata & \nodata\\
HD 102117 b & 325254372 & 0.046$^{+0.007}_{-0.006}$ & 0.046$^{+0.007}_{-0.006}$ & 10,11 & 2,3 & \nodata & \nodata\\
mu Leo b & 73416947 & 0.046$^{+0.005}_{-0.004}$ & 0.0035$^{+0.0004}_{-0.0003}$ & \nodata & \nodata & 8 & 1\\
GJ 273 c & 178872239 & 0.046$^{+0.01}_{-0.007}$ & 0.046$^{+0.01}_{-0.007}$ & 7 & 1 & \nodata & \nodata\\
HD 173416 b & 265052133 & 0.046$^{+0.004}_{-0.004}$ & 0.0038$^{+0.0004}_{-0.0003}$ & \nodata & \nodata & 13 & 3\\
HD 99492 b & 49427341 & 0.046$^{+0.009}_{-0.007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 190360 c & 105999792 & 0.045$^{+0.006}_{-0.005}$ & 0.045$^{+0.006}_{-0.005}$ & \nodata & \nodata & 1 & 2\\
HD 97658 b & 363549734 & 0.045$^{+0.004}_{-0.003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 224693 b & 37947783 & 0.044$^{+0.009}_{-0.008}$ & 0.044$^{+0.009}_{-0.008}$ & 2 & 1 & \nodata & \nodata\\
HD 125595 b & 61397572 & 0.044$^{+0.006}_{-0.005}$ & 0.044$^{+0.006}_{-0.005}$ & 11 & 1 & \nodata & \nodata\\
gam Lib b & 386935627 & 0.044$^{+0.008}_{-0.006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 433 b & 118608254 & 0.044$^{+0.008}_{-0.006}$ & 0.044$^{+0.008}_{-0.006}$ & 10 & 2 & \nodata & \nodata\\
55 Cnc b & 21535479 & 0.0431$^{+0.001}_{-0.0009}$ & 0.0431$^{+0.001}_{-0.0009}$ & \nodata & \nodata & 7 & 1\\
GJ 163 b & 35725282 & 0.043$^{+0.005}_{-0.005}$ & 0.043$^{+0.005}_{-0.005}$ & 3,4,5 & 3,3,3 & \nodata & \nodata\\
HD 20794 b & 301051051 & 0.042$^{+0.006}_{-0.006}$ & 0.042$^{+0.006}_{-0.006}$ & 3,4 & 3,3 & \nodata & \nodata\\
GJ 667 C b & 236743275 & 0.042$^{+0.009}_{-0.007}$ & 0.042$^{+0.009}_{-0.007}$ & 12 & 1 & \nodata & \nodata\\
YZ Cet c & 423862056 & 0.042$^{+0.006}_{-0.005}$ & 0.042$^{+0.006}_{-0.005}$ & 3 & 1 & \nodata & \nodata\\
HD 177830 c & 392658786 & 0.041$^{+0.007}_{-0.005}$ & 0.01$^{+0.002}_{-0.001}$ & \nodata & \nodata & 13 & 2\\
HD 4308 b & 234501204 & 0.041$^{+0.005}_{-0.004}$ & 0.041$^{+0.005}_{-0.004}$ & 1,2 & 3,3 & \nodata & \nodata\\
HD 108147 b & 371621238 & 0.04$^{+0.01}_{-0.009}$ & 0.04$^{+0.01}_{-0.009}$ & 11 & 2 & \nodata & \nodata\\
HD 215152 d & 251042502 & 0.039$^{+0.001}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 10180 d & 231836962 & 0.039$^{+0.002}_{-0.002}$ & 0.039$^{+0.002}_{-0.002}$ & 1,2 & 3,3 & \nodata & \nodata\\
eps Tau b & 17554529 & 0.039$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 86 b & 284181945 & 0.039$^{+0.004}_{-0.004}$ & 0.039$^{+0.004}_{-0.004}$ & 2,3 & 3,3 & \nodata & \nodata\\
nu Oph b & 68984421 & 0.039$^{+0.005}_{-0.004}$ & 0.002$^{+0.0003}_{-0.0002}$ & \nodata & \nodata & 13 & 1\\
HD 168443 b & 53134037 & 0.038$^{+0.002}_{-0.002}$ & 0.0177$^{+0.0007}_{-0.0007}$ & \nodata & \nodata & 13 & 1\\
GJ 581 b & 138819293 & 0.04$^{+0.02}_{-0.02}$ & 0.04$^{+0.02}_{-0.02}$ & \nodata & \nodata & 11 & 1\\
HD 240210 b & 397354290 & 0.037$^{+0.007}_{-0.007}$ & 0.004$^{+0.0008}_{-0.0007}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 69830 c & 73312938 & 0.04$^{+0.04}_{-0.04}$ & 0.03$^{+0.03}_{-0.03}$ & 7 & 2 & \nodata & \nodata\\
HD 14067 b & 37748347 & 0.036$^{+0.005}_{-0.005}$ & 0.00066$^{+0.00009}_{-0.00008}$ & \nodata & \nodata & 4 & 1\\
HD 180314 b & 410399074 & 0.035$^{+0.002}_{-0.002}$ & 0.0048$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & 1,13 & 3,3\\
IC 4651 9122 b & 214416505 & 0.04$^{+0.01}_{-0.01}$ & 0.0013$^{+0.0004}_{-0.0004}$ & 12 & 1 & \nodata & \nodata\\
HD 45652 b & 206948365 & 0.035$^{+0.006}_{-0.005}$ & 0.022$^{+0.004}_{-0.003}$ & 6 & 1 & \nodata & \nodata\\
HD 156279 b & 165987272 & 0.035$^{+0.003}_{-0.002}$ & 0.035$^{+0.003}_{-0.002}$ & \nodata & \nodata & 1,2,3,4,5,6,7,8,9,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4,4\\
YZ Cet d & 284907742 & 0.035$^{+0.005}_{-0.004}$ & 0.035$^{+0.005}_{-0.004}$ & 3 & 1 & \nodata & \nodata\\
GJ 536 b & 119147875 & 0.034$^{+0.004}_{-0.004}$ & 0.034$^{+0.004}_{-0.004}$ & \nodata & \nodata & 10 & 1\\
HD 7924 c & 468723402 & 0.034$^{+0.004}_{-0.002}$ & 0.034$^{+0.004}_{-0.002}$ & \nodata & \nodata & 5 & 3\\
HD 27894 b & 396697266 & 0.034$^{+0.001}_{-0.001}$ & 0.034$^{+0.001}_{-0.001}$ & 1,2,3,4,5,8,9,11,12 & 4,4,3,3,4,4,4,4,4 & \nodata & \nodata\\
tau Cet h & 439403362 & 0.03$^{+0.04}_{-0.03}$ & 0.02$^{+0.02}_{-0.02}$ & 3 & 1 & \nodata & \nodata\\
HD 285968 b & 176379354 & 0.034$^{+0.004}_{-0.003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 175541 b & 137121812 & 0.033$^{+0.01}_{-0.008}$ & 0.003$^{+0.001}_{-0.0007}$ & \nodata & \nodata & 13 & 1\\
HD 74156 b & 21285884 & 0.033$^{+0.001}_{-0.001}$ & 0.0174$^{+0.0007}_{-0.0007}$ & 7 & 1 & \nodata & \nodata\\
HD 110014 b & 292113181 & 0.033$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 3341 b & 405485269 & 0.033$^{+0.007}_{-0.005}$ & 0.033$^{+0.007}_{-0.005}$ & 5,6 & 3,3 & \nodata & \nodata\\
HD 40307 d & 374859347 & 0.033$^{+0.007}_{-0.006}$ & 0.033$^{+0.007}_{-0.006}$ & 1,2,3,4,5,6,7,8,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4 & \nodata & \nodata\\
HD 102329 b & 96195878 & 0.032$^{+0.003}_{-0.003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 176986 c & 39554091 & 0.032$^{+0.004}_{-0.003}$ & 0.032$^{+0.004}_{-0.003}$ & \nodata & \nodata & 13 & 1\\
70 Vir b & 422478973 & 0.0315$^{+0.0009}_{-0.0009}$ & 0.0073$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 10 & 1\\
HD 109271 c & 422214062 & 0.031$^{+0.006}_{-0.005}$ & 0.027$^{+0.005}_{-0.004}$ & 10 & 1 & \nodata & \nodata\\
HD 177565 b & 328997091 & 0.03$^{+0.03}_{-0.03}$ & 0.02$^{+0.02}_{-0.02}$ & 13 & 1 & \nodata & \nodata\\
Kepler-432 c & 22874788 & 0.031$^{+0.003}_{-0.003}$ & 0.0062$^{+0.0005}_{-0.0006}$ & \nodata & \nodata & 1,2,13 & 3,3,3\\
rho CrB b & 458494003 & 0.0303$^{+0.0008}_{-0.0008}$ & 0.0205$^{+0.0006}_{-0.0005}$ & \nodata & \nodata & 11 & 2\\
HD 28678 b & 449145115 & 0.03$^{+0.004}_{-0.003}$ & 0.0021$^{+0.0002}_{-0.0002}$ & 5 & 1 & \nodata & \nodata\\
GJ 3293 e & 122375047 & 0.03$^{+0.01}_{-0.005}$ & 0.03$^{+0.01}_{-0.005}$ & 5 & 2 & \nodata & \nodata\\
HD 219134 f & 49064384 & 0.03$^{+0.002}_{-0.002}$ & 0.03$^{+0.002}_{-0.002}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 47366 b & 443578538 & 0.03$^{+0.003}_{-0.002}$ & 0.0022$^{+0.0002}_{-0.0002}$ & 6 & 2 & \nodata & \nodata\\
HD 72892 b & 405344271 & 0.029$^{+0.002}_{-0.002}$ & 0.02$^{+0.001}_{-0.001}$ & 8 & 2 & \nodata & \nodata\\
HD 154672 b & 21897561 & 0.029$^{+0.003}_{-0.002}$ & 0.0047$^{+0.0004}_{-0.0004}$ & 12 & 2 & \nodata & \nodata\\
HD 192263 b & 243962745 & 0.028$^{+0.004}_{-0.003}$ & 0.028$^{+0.004}_{-0.003}$ & \nodata & \nodata & 1 & 1\\
GJ 3998 c & 369021303 & 0.028$^{+0.003}_{-0.003}$ & 0.028$^{+0.003}_{-0.003}$ & \nodata & \nodata & 12 & 2\\
HIP 65407 b & 156067565 & 0.028$^{+0.005}_{-0.004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 40956 b & 435907158 & 0.028$^{+0.003}_{-0.002}$ & 0.0013$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 6 & 2\\
HD 120084 b & 347909637 & 0.028$^{+0.02}_{-0.007}$ & 0.0011$^{+0.0007}_{-0.0003}$ & \nodata & \nodata & 6,7,8 & 3,3,3\\
HD 11977 b & 232074535 & 0.028$^{+0.004}_{-0.003}$ & 0.0021$^{+0.0003}_{-0.0003}$ & 1,2 & 3,3 & \nodata & \nodata\\
HD 16141 b & 251109533 & 0.027$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 147873 b & 211080657 & 0.027$^{+0.002}_{-0.001}$ & 0.0062$^{+0.0004}_{-0.0003}$ & 12 & 1 & \nodata & \nodata\\
HD 43691 b & 26817004 & 0.027$^{+0.005}_{-0.004}$ & 0.019$^{+0.004}_{-0.003}$ & \nodata & \nodata & 6 & 1\\
Kepler-20 g & 290172418 & 0.026$^{+0.002}_{-0.002}$ & 0.026$^{+0.002}_{-0.002}$ & \nodata & \nodata & 1,13 & 3,3\\
HD 9446 b & 18277196 & 0.03$^{+0.01}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 7924 d & 405485269 & 0.026$^{+0.006}_{-0.003}$ & 0.026$^{+0.006}_{-0.003}$ & \nodata & \nodata & 5 & 3\\
HD 114762 b & 217831699 & 0.0257$^{+0.0009}_{-0.0009}$ & 0.0083$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & 10 & 1\\
gam Lib c & 386935627 & 0.025$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 20794 c & 356473029 & 0.025$^{+0.003}_{-0.003}$ & 0.025$^{+0.003}_{-0.003}$ & 3,4 & 3,3 & \nodata & \nodata\\
HD 4732 b & 63905972 & 0.025$^{+0.003}_{-0.003}$ & 0.0019$^{+0.0002}_{-0.0002}$ & 3 & 1 & \nodata & \nodata\\
TYC 1422-614-1 c & 459558974 & 0.025$^{+0.005}_{-0.005}$ & 0.0012$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 8 & 1\\
HD 34445 e & 302372658 & 0.025$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
75 Cet b & 66914642 & 0.025$^{+0.004}_{-0.003}$ & 0.001$^{+0.0002}_{-0.0001}$ & 4 & 1 & \nodata & \nodata\\
GJ 3323 b & 43605290 & 0.024$^{+0.007}_{-0.006}$ & 0.024$^{+0.007}_{-0.006}$ & 5 & 1 & \nodata & \nodata\\
HD 47366 c & 443578538 & 0.024$^{+0.003}_{-0.003}$ & 0.0009$^{+0.0001}_{-0.0001}$ & 6 & 2 & \nodata & \nodata\\
HD 62509 b & 423088367 & 0.024$^{+0.005}_{-0.003}$ & 0.0011$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 7 & 1\\
HD 90156 b & 53178442 & 0.024$^{+0.004}_{-0.003}$ & 0.013$^{+0.002}_{-0.002}$ & 9 & 2 & \nodata & \nodata\\
HIP 57274 c & 200385493 & 0.024$^{+0.003}_{-0.003}$ & 0.02$^{+0.003}_{-0.002}$ & \nodata & \nodata & 9 & 1\\
HD 96167 b & 38158652 & 0.023$^{+0.004}_{-0.003}$ & 0.0013$^{+0.0002}_{-0.0002}$ & 9 & 1 & \nodata & \nodata\\
HD 108863 b & 113810736 & 0.023$^{+0.001}_{-0.001}$ & 0.00143$^{+0.00008}_{-0.00008}$ & \nodata & \nodata & 9 & 1\\
HD 107148 b & 437258837 & 0.02$^{+0.01}_{-0.01}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 204313 c & 405501056 & 0.023$^{+0.002}_{-0.002}$ & 0.018$^{+0.001}_{-0.001}$ & 1 & 1 & \nodata & \nodata\\
HD 208897 b & 284907742 & 0.023$^{+0.002}_{-0.002}$ & 0.0017$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 2 & 1\\
HD 215152 e & 251042502 & 0.0225$^{+0.0007}_{-0.0007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
81 Cet b & 95473936 & 0.022$^{+0.004}_{-0.003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 147018 b & 350673608 & 0.022$^{+0.001}_{-0.001}$ & 0.0136$^{+0.0007}_{-0.0007}$ & 12 & 2 & \nodata & \nodata\\
Ross 128 b & 325275315 & 0.022$^{+0.003}_{-0.003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 99706 b & 4610441 & 0.022$^{+0.004}_{-0.003}$ & 0.0007$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 8 & 2\\
HD 171028 b & 398943781 & 0.022$^{+0.001}_{-0.001}$ & 0.00109$^{+0.00005}_{-0.00005}$ & \nodata & \nodata & 13 & 2\\
HD 96063 b & 437246853 & 0.0218$^{+0.001}_{-0.0009}$ & 0.00163$^{+0.00007}_{-0.00007}$ & 9 & 1 & \nodata & \nodata\\
HD 175607 b & 283722336 & 0.022$^{+0.002}_{-0.001}$ & 0.02$^{+0.002}_{-0.001}$ & 13 & 2 & \nodata & \nodata\\
HD 4313 b & 117768715 & 0.022$^{+0.001}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 210702 b & 277774779 & 0.022$^{+0.003}_{-0.003}$ & 0.0016$^{+0.0003}_{-0.0002}$ & \nodata & \nodata & 2 & 1\\
HD 164595 b & 220017951 & 0.022$^{+0.004}_{-0.003}$ & 0.022$^{+0.004}_{-0.003}$ & \nodata & \nodata & 12,13 & 3,2\\
TYC 3318-01333-1 b & 116376087 & 0.021$^{+0.004}_{-0.004}$ & 0.001$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 5 & 2\\
HD 148427 b & 173552927 & 0.021$^{+0.002}_{-0.002}$ & 0.0017$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 12 & 1\\
HD 139357 b & 119974993 & 0.021$^{+0.002}_{-0.002}$ & 0.0015$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 9,10,11 & 3,3,3\\
HD 192699 b & 27864699 & 0.021$^{+0.002}_{-0.001}$ & 0.0017$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 1 & 1\\
HD 212771 b & 12723961 & 0.021$^{+0.002}_{-0.002}$ & 0.0015$^{+0.0001}_{-0.0001}$ & 2 & 1 & \nodata & \nodata\\
61 Vir c & 422478973 & 0.021$^{+0.002}_{-0.002}$ & 0.015$^{+0.001}_{-0.001}$ & 10 & 1 & \nodata & \nodata\\
HD 10180 e & 231836962 & 0.02$^{+0.001}_{-0.001}$ & 0.02$^{+0.001}_{-0.001}$ & 1,2 & 3,3 & \nodata & \nodata\\
HD 111591 b & 158554588 & 0.02$^{+0.003}_{-0.003}$ & 0.00052$^{+0.00009}_{-0.00007}$ & \nodata & \nodata & 9 & 1\\
HD 158038 b & 57983992 & 0.02$^{+0.003}_{-0.002}$ & 0.001$^{+0.0002}_{-0.0001}$ & \nodata & \nodata & 12 & 2\\
GJ 581 c & 36853511 & 0.02$^{+0.01}_{-0.009}$ & 0.02$^{+0.01}_{-0.009}$ & \nodata & \nodata & 11 & 1\\
HD 33142 b & 169397663 & 0.02$^{+0.005}_{-0.003}$ & 0.0016$^{+0.0004}_{-0.0003}$ & 5 & 2 & \nodata & \nodata\\
HD 27894 c & 396697266 & 0.0198$^{+0.0008}_{-0.0007}$ & 0.0198$^{+0.0008}_{-0.0007}$ & 1,2,3,4,5,8,9,11,12 & 4,4,3,3,4,4,4,4,4 & \nodata & \nodata\\
HD 206610 b & 283621278 & 0.02$^{+0.002}_{-0.002}$ & 0.00088$^{+0.0001}_{-0.00009}$ & \nodata & \nodata & 1 & 1\\
HIP 67537 b & 396697266 & 0.02$^{+0.003}_{-0.002}$ & 0.00021$^{+0.00003}_{-0.00003}$ & 11 & 1 & \nodata & \nodata\\
HD 52265 b & 200658785 & 0.02$^{+0.002}_{-0.002}$ & 0.0045$^{+0.0005}_{-0.0004}$ & 7 & 1 & \nodata & \nodata\\
55 Cnc c & 332064670 & 0.0197$^{+0.0008}_{-0.0006}$ & 0.012$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & 7 & 1\\
GJ 876 c & 178872239 & 0.019$^{+0.007}_{-0.007}$ & 0.017$^{+0.006}_{-0.006}$ & 2 & 1 & \nodata & \nodata\\
HD 26965 b & 67772871 & 0.019$^{+0.004}_{-0.004}$ & 0.012$^{+0.002}_{-0.002}$ & 5 & 1 & \nodata & \nodata\\
Wolf 1061 c & 413948621 & 0.019$^{+0.003}_{-0.002}$ & 0.019$^{+0.003}_{-0.002}$ & \nodata & \nodata & 12 & 1\\
GJ 163 c & 219221189 & 0.019$^{+0.003}_{-0.003}$ & 0.019$^{+0.003}_{-0.003}$ & 3,4,5 & 3,3,3 & \nodata & \nodata\\
HD 109246 b & 329649885 & 0.019$^{+0.001}_{-0.001}$ & 0.0151$^{+0.0009}_{-0.0009}$ & \nodata & \nodata & 7,8 & 3,3\\
HD 3651 b & 434210589 & 0.02$^{+0.02}_{-0.02}$ & 0.008$^{+0.008}_{-0.008}$ & \nodata & \nodata & 3 & 1\\
GJ 625 b & 284907742 & 0.019$^{+0.004}_{-0.004}$ & 0.019$^{+0.004}_{-0.004}$ & \nodata & \nodata & 9,10,11,12 & 3,3,3,3\\
HD 33844 b & 169534187 & 0.019$^{+0.002}_{-0.002}$ & 0.00092$^{+0.0001}_{-0.00009}$ & 5 & 2 & \nodata & \nodata\\
HD 136418 b & 172607132 & 0.019$^{+0.001}_{-0.001}$ & 0.0022$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 10,11 & 3,3\\
omi UMa b & 189576919 & 0.019$^{+0.003}_{-0.002}$ & 0.00031$^{+0.00005}_{-0.00004}$ & \nodata & \nodata & 7 & 2\\
HD 178911 B b & 410399074 & 0.018$^{+0.001}_{-0.001}$ & 0.0139$^{+0.0008}_{-0.0007}$ & \nodata & \nodata & 1,13 & 3,3\\
GJ 832 c & 188580272 & 0.02$^{+0.01}_{-0.01}$ & 0.014$^{+0.008}_{-0.008}$ & 1 & 2 & \nodata & \nodata\\
24 Sex b & 354489950 & 0.018$^{+0.002}_{-0.001}$ & 0.00105$^{+0.0001}_{-0.00008}$ & 8 & 1 & \nodata & \nodata\\
HD 167042 b & 321030607 & 0.017$^{+0.001}_{-0.001}$ & 0.0112$^{+0.0007}_{-0.0007}$ & \nodata & \nodata & 1,2,4,5,7,8,9,11,12,13 & 4,4,4,4,4,4,4,4,4,3\\
HD 145377 b & 312545949 & 0.0174$^{+0.0008}_{-0.0007}$ & 0.0045$^{+0.0002}_{-0.0002}$ & 12 & 1 & \nodata & \nodata\\
HD 103197 b & 160224839 & 0.017$^{+0.002}_{-0.002}$ & 0.01$^{+0.001}_{-0.001}$ & 10 & 2 & \nodata & \nodata\\
GJ 273 b & 318686860 & 0.017$^{+0.003}_{-0.002}$ & 0.017$^{+0.003}_{-0.002}$ & 7 & 1 & \nodata & \nodata\\
HD 121504 b & 287973473 & 0.0173$^{+0.0007}_{-0.0007}$ & 0.0074$^{+0.0003}_{-0.0003}$ & 11 & 2 & \nodata & \nodata\\
HD 20868 b & 142851295 & 0.017$^{+0.001}_{-0.001}$ & 0.00122$^{+0.00008}_{-0.00008}$ & 4 & 2 & \nodata & \nodata\\
HIP 12961 b & 204614039 & 0.017$^{+0.002}_{-0.002}$ & 0.0081$^{+0.0009}_{-0.0008}$ & 4 & 2 & \nodata & \nodata\\
HD 208487 b & 197686484 & 0.017$^{+0.01}_{-0.008}$ & 0.004$^{+0.002}_{-0.002}$ & 1 & 1 & \nodata & \nodata\\
HD 60532 b & 456871289 & 0.017$^{+0.001}_{-0.001}$ & 0.0023$^{+0.0001}_{-0.0001}$ & 7 & 2 & \nodata & \nodata\\
HD 82886 b & 62760824 & 0.017$^{+0.004}_{-0.003}$ & 0.0007$^{+0.0002}_{-0.0001}$ & \nodata & \nodata & 8 & 1\\
HD 216770 b & 405688133 & 0.017$^{+0.002}_{-0.002}$ & 0.0039$^{+0.0004}_{-0.0004}$ & 2 & 1 & \nodata & \nodata\\
GJ 676 A e & 220408612 & 0.017$^{+0.003}_{-0.003}$ & 0.013$^{+0.002}_{-0.002}$ & 12 & 1 & \nodata & \nodata\\
HD 164922 c & 159019691 & 0.017$^{+0.003}_{-0.002}$ & 0.012$^{+0.002}_{-0.002}$ & \nodata & \nodata & 12,13 & 2,2\\
HD 40307 f & 374859347 & 0.017$^{+0.003}_{-0.003}$ & 0.017$^{+0.003}_{-0.003}$ & 1,2,3,4,5,6,7,8,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4 & \nodata & \nodata\\
GJ 667 C c & 369021303 & 0.017$^{+0.003}_{-0.003}$ & 0.016$^{+0.003}_{-0.002}$ & 12 & 1 & \nodata & \nodata\\
HD 101930 b & 32820141 & 0.0167$^{+0.001}_{-0.0009}$ & 0.0128$^{+0.0008}_{-0.0007}$ & 10,11 & 2,2 & \nodata & \nodata\\
HD 219134 d & 417676622 & 0.0166$^{+0.0006}_{-0.0005}$ & 0.0166$^{+0.0006}_{-0.0005}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 181342 b & 112243062 & 0.017$^{+0.002}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 154857 b & 412409409 & 0.0162$^{+0.0008}_{-0.0007}$ & 0.00107$^{+0.00005}_{-0.00005}$ & 12 & 2 & \nodata & \nodata\\
HD 18742 b & 71345433 & 0.016$^{+0.001}_{-0.001}$ & 0.00056$^{+0.00005}_{-0.00005}$ & 4 & 2 & \nodata & \nodata\\
HD 222582 b & 9005067 & 0.016$^{+0.0008}_{-0.0007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
tau Cet e & 439403362 & 0.02$^{+0.02}_{-0.02}$ & 0.003$^{+0.003}_{-0.003}$ & 3 & 1 & \nodata & \nodata\\
rho CrB c & 458494003 & 0.0159$^{+0.0009}_{-0.0008}$ & 0.0042$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 11 & 2\\
18 Del b & 27533327 & 0.016$^{+0.008}_{-0.008}$ & 0.0004$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 1 & 1\\
HD 1502 b & 303193565 & 0.0156$^{+0.0007}_{-0.0007}$ & 0.00098$^{+0.00005}_{-0.00005}$ & \nodata & \nodata & 3 & 1\\
GJ 3293 b & 105438311 & 0.015$^{+0.001}_{-0.001}$ & 0.014$^{+0.001}_{-0.001}$ & 5 & 2 & \nodata & \nodata\\
HD 169830 b & 227196910 & 0.015$^{+0.008}_{-0.007}$ & 0.0018$^{+0.0009}_{-0.0009}$ & 13 & 1 & \nodata & \nodata\\
HD 152581 b & 173552927 & 0.015$^{+0.001}_{-0.001}$ & 0.0006$^{+0.00004}_{-0.00004}$ & \nodata & \nodata & 12 & 2\\
HD 177830 b & 2288734 & 0.015$^{+0.001}_{-0.001}$ & 0.00101$^{+0.00008}_{-0.00007}$ & \nodata & \nodata & 13 & 2\\
HIP 65407 c & 366659915 & 0.015$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 141399 b & 419015728 & 0.015$^{+0.001}_{-0.001}$ & 0.0087$^{+0.0007}_{-0.0006}$ & \nodata & \nodata & 10,11 & 3,3\\
HD 1605 b & 57983992 & 0.015$^{+0.001}_{-0.001}$ & 0.00071$^{+0.00006}_{-0.00005}$ & \nodata & \nodata & 3 & 1\\
HIP 65891 b & 42812945 & 0.015$^{+0.002}_{-0.002}$ & 0.00038$^{+0.00005}_{-0.00005}$ & 11 & 2 & \nodata & \nodata\\
HD 5608 b & 53873088 & 0.015$^{+0.001}_{-0.001}$ & 0.00051$^{+0.00005}_{-0.00004}$ & \nodata & \nodata & 4 & 1\\
HD 131496 b & 402802683 & 0.015$^{+0.002}_{-0.001}$ & 0.00045$^{+0.00005}_{-0.00004}$ & \nodata & \nodata & 11 & 2\\
HD 95089 b & 19028197 & 0.015$^{+0.002}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 20794 d & 301051051 & 0.015$^{+0.002}_{-0.002}$ & 0.009$^{+0.001}_{-0.001}$ & 3,4 & 3,3 & \nodata & \nodata\\
HD 86950 b & 332711151 & 0.015$^{+0.002}_{-0.002}$ & 0.00062$^{+0.0001}_{-0.00009}$ & 8,9 & 1,1 & \nodata & \nodata\\
HD 85512 b & 407591082 & 0.015$^{+0.003}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 104067 b & 176940023 & 0.015$^{+0.002}_{-0.001}$ & 0.0071$^{+0.0009}_{-0.0007}$ & 10 & 1 & \nodata & \nodata\\
HD 73526 b & 11749208 & 0.0146$^{+0.001}_{-0.0009}$ & 0.0042$^{+0.0003}_{-0.0003}$ & 8,9 & 3,3 & \nodata & \nodata\\
Kepler-19 d & 166526615 & 0.0145$^{+0.002}_{-0.0009}$ & 0.0124$^{+0.001}_{-0.0007}$ & \nodata & \nodata & 1,13 & 3,3\\
HD 180902 b & 48777312 & 0.014$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 30562 b & 13147218 & 0.014$^{+0.004}_{-0.003}$ & 0.00034$^{+0.00009}_{-0.00006}$ & 5 & 1 & \nodata & \nodata\\
HD 231701 b & 92300251 & 0.014$^{+0.002}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 200964 b & 408316773 & 0.0142$^{+0.0008}_{-0.0008}$ & 0.00063$^{+0.00004}_{-0.00003}$ & \nodata & \nodata & 1 & 1\\
HD 102365 b & 229137615 & 0.014$^{+0.009}_{-0.008}$ & 0.003$^{+0.002}_{-0.002}$ & 10 & 2 & \nodata & \nodata\\
HD 116029 b & 208844024 & 0.0141$^{+0.0007}_{-0.0007}$ & 0.00057$^{+0.00003}_{-0.00003}$ & \nodata & \nodata & 10 & 2\\
HD 98219 b & 148680230 & 0.014$^{+0.0006}_{-0.0006}$ & 0.00086$^{+0.00004}_{-0.00004}$ & 9 & 1 & \nodata & \nodata\\
HD 34445 d & 284907742 & 0.0139$^{+0.0006}_{-0.0006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 12484 b & 156067565 & 0.0138$^{+0.001}_{-0.0009}$ & 0.0063$^{+0.0005}_{-0.0004}$ & 4 & 1 & \nodata & \nodata\\
GJ 687 b & 188580272 & 0.014$^{+0.002}_{-0.002}$ & 0.014$^{+0.002}_{-0.002}$ & \nodata & \nodata & 2,3,4,5,6,7,8,9,10,12,13 & 4,4,4,4,4,4,4,4,4,4,4\\
GJ 667 C f & 369021303 & 0.013$^{+0.002}_{-0.002}$ & 0.009$^{+0.002}_{-0.001}$ & 12 & 1 & \nodata & \nodata\\
HD 155358 b & 257715493 & 0.0134$^{+0.0007}_{-0.0007}$ & 0.00186$^{+0.0001}_{-0.00009}$ & \nodata & \nodata & 12 & 3\\
HD 8574 b & 18121498 & 0.0131$^{+0.0007}_{-0.0006}$ & 0.00156$^{+0.00008}_{-0.00007}$ & \nodata & \nodata & 4 & 1\\
HIP 74890 b & 148153804 & 0.013$^{+0.002}_{-0.002}$ & 0.00043$^{+0.00006}_{-0.00005}$ & 11 & 1 & \nodata & \nodata\\
HD 192310 b & 326096771 & 0.013$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 82943 c & 35055332 & 0.013$^{+0.006}_{-0.006}$ & 0.0016$^{+0.0008}_{-0.0008}$ & 8 & 1 & \nodata & \nodata\\
HD 35759 b & 419940916 & 0.0129$^{+0.0007}_{-0.0007}$ & 0.0042$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 6 & 2\\
Kepler-25 d & 286954708 & 0.0129$^{+0.0005}_{-0.0004}$ & 0.0056$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 1,13 & 3,3\\
HD 4203 b & 434225151 & 0.0128$^{+0.001}_{-0.0009}$ & 0.0008$^{+0.00006}_{-0.00006}$ & \nodata & \nodata & 3 & 1\\
24 Sex c & 21535479 & 0.013$^{+0.004}_{-0.003}$ & 0.0004$^{+0.0001}_{-0.0001}$ & 8 & 1 & \nodata & \nodata\\
HD 30856 b & 612908 & 0.013$^{+0.003}_{-0.002}$ & 0.00037$^{+0.0001}_{-0.00007}$ & 5 & 2 & \nodata & \nodata\\
HD 38283 b & 141411201 & 0.012$^{+0.005}_{-0.003}$ & 0.01$^{+0.004}_{-0.002}$ & 1,2,4,5,6,7,8,9,10,11,12 & 4,4,4,4,4,4,4,4,4,4,4 & \nodata & \nodata\\
HD 33844 c & 169534187 & 0.012$^{+0.002}_{-0.001}$ & 0.00036$^{+0.00005}_{-0.00004}$ & 5 & 2 & \nodata & \nodata\\
HD 69830 d & 307624961 & 0.01$^{+0.01}_{-0.01}$ & 0.002$^{+0.002}_{-0.002}$ & 7 & 2 & \nodata & \nodata\\
HD 5319 b & 278380701 & 0.0123$^{+0.0007}_{-0.0006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 155233 b & 399334674 & 0.012$^{+0.001}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 128356 b & 16855 & 0.012$^{+0.003}_{-0.002}$ & 0.0011$^{+0.0003}_{-0.0002}$ & 11 & 1 & \nodata & \nodata\\
nu Oph c & 9815387 & 0.012$^{+0.002}_{-0.001}$ & 0.0001$^{+0.00001}_{-0.00001}$ & \nodata & \nodata & 13 & 1\\
HD 7449 b & 248381971 & 0.012$^{+0.006}_{-0.003}$ & 0.00026$^{+0.0001}_{-0.00006}$ & 3 & 1 & \nodata & \nodata\\
Proxima Cen b & 369021303 & 0.012$^{+0.002}_{-0.002}$ & 0.012$^{+0.002}_{-0.002}$ & 11,12 & 2,2 & \nodata & \nodata\\
HAT-P-13 c & 231836962 & 0.0119$^{+0.0007}_{-0.0006}$ & 0.00072$^{+0.00004}_{-0.00004}$ & \nodata & \nodata & 7 & 1\\
gam Cep b & 272677041 & 0.012$^{+0.006}_{-0.006}$ & 0.0004$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 5 & 3\\
HD 44219 b & 443055162 & 0.012$^{+0.003}_{-0.002}$ & 0.0007$^{+0.0001}_{-0.0001}$ & 6 & 2 & \nodata & \nodata\\
HD 200964 c & 408316773 & 0.012$^{+0.002}_{-0.002}$ & 0.00039$^{+0.00006}_{-0.00006}$ & \nodata & \nodata & 1 & 1\\
HD 12661 b & 224312054 & 0.0118$^{+0.0004}_{-0.0004}$ & 0.00121$^{+0.00004}_{-0.00004}$ & \nodata & \nodata & 4 & 1\\
GJ 3293 d & 178872239 & 0.012$^{+0.002}_{-0.001}$ & 0.0065$^{+0.001}_{-0.0008}$ & 5 & 2 & \nodata & \nodata\\
HIP 8541 b & 231019255 & 0.012$^{+0.002}_{-0.002}$ & 0.0004$^{+0.00007}_{-0.00006}$ & 2,3 & 3,3 & \nodata & \nodata\\
16 Cyg B b & 219483057 & 0.011$^{+0.0008}_{-0.0007}$ & 0.00074$^{+0.00005}_{-0.00005}$ & \nodata & \nodata & 1,2 & 3,3\\
HD 93083 b & 286277386 & 0.011$^{+0.003}_{-0.002}$ & 0.0021$^{+0.0005}_{-0.0004}$ & 9 & 2 & \nodata & \nodata\\
6 Lyn b & 251095345 & 0.011$^{+0.001}_{-0.001}$ & 0.00033$^{+0.00005}_{-0.00003}$ & \nodata & \nodata & 6 & 2\\
HD 10442 b & 380908091 & 0.0108$^{+0.0009}_{-0.0008}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
BD+49 828 b & 397024052 & 0.011$^{+0.004}_{-0.003}$ & 0.00011$^{+0.00005}_{-0.00003}$ & \nodata & \nodata & 5 & 2\\
GJ 1148 b & 115869504 & 0.011$^{+0.004}_{-0.004}$ & 0.007$^{+0.003}_{-0.003}$ & \nodata & \nodata & 8 & 2\\
HD 10180 f & 231836962 & 0.0105$^{+0.0007}_{-0.0007}$ & 0.0046$^{+0.0003}_{-0.0003}$ & 1,2 & 3,3 & \nodata & \nodata\\
HD 222076 b & 325178933 & 0.01$^{+0.002}_{-0.002}$ & 0.00032$^{+0.00005}_{-0.00005}$ & 1 & 3 & \nodata & \nodata\\
HD 207832 b & 53895723 & 0.01$^{+0.002}_{-0.001}$ & 0.0017$^{+0.0003}_{-0.0002}$ & 1 & 1 & \nodata & \nodata\\
HD 142415 b & 350083732 & 0.0102$^{+0.0003}_{-0.0003}$ & 0.00071$^{+0.00002}_{-0.00002}$ & 12 & 2 & \nodata & \nodata\\
HD 42618 b & 153289168 & 0.01$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 16175 b & 422922274 & 0.01$^{+0.004}_{-0.002}$ & 0.00027$^{+0.0001}_{-0.00006}$ & \nodata & \nodata & 4 & 1\\
30 Ari B b & 139298196 & 0.01$^{+0.002}_{-0.001}$ & 0.0008$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 4 & 1\\
HD 219134 g & 302069358 & 0.01$^{+0.0002}_{-0.0002}$ & 0.0058$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 147873 c & 211080657 & 0.01$^{+0.0007}_{-0.0007}$ & 0.00055$^{+0.00004}_{-0.00004}$ & 12 & 1 & \nodata & \nodata\\
HD 134987 b & 437430894 & 0.01$^{+0.0004}_{-0.0004}$ & 0.00105$^{+0.00004}_{-0.00004}$ & 11 & 1 & \nodata & \nodata\\
HD 31253 b & 144730053 & 0.01$^{+0.004}_{-0.002}$ & 0.0006$^{+0.0002}_{-0.0001}$ & 5 & 1 & \nodata & \nodata\\
GJ 667 C e & 188580272 & 0.01$^{+0.002}_{-0.002}$ & 0.0042$^{+0.0008}_{-0.0007}$ & 12 & 1 & \nodata & \nodata\\
HD 89744 b & 252794572 & 0.0098$^{+0.0003}_{-0.0003}$ & 0.00103$^{+0.00003}_{-0.00003}$ & \nodata & \nodata & 8 & 1\\
HD 238914 b & 359558085 & 0.01$^{+0.004}_{-0.003}$ & 0.0008$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & 1,2,3,4,5,6,7,8,9,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4,4\\
HD 40979 b & 440489582 & 0.0097$^{+0.0003}_{-0.0003}$ & 0.00099$^{+0.00003}_{-0.00003}$ & \nodata & \nodata & 6 & 1\\
GJ 876 b & 63905972 & 0.01$^{+0.003}_{-0.003}$ & 0.004$^{+0.002}_{-0.002}$ & 2 & 1 & \nodata & \nodata\\
HD 34445 c & 284907742 & 0.0095$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
XO-2 S c & 469943599 & 0.0095$^{+0.0004}_{-0.0004}$ & 0.00213$^{+0.0001}_{-0.00009}$ & \nodata & \nodata & 7 & 1\\
HD 2039 b & 281461362 & 0.01$^{+0.002}_{-0.001}$ & 0.00046$^{+0.0001}_{-0.00007}$ & 1,2 & 2,2 & \nodata & \nodata\\
HD 40307 g & 434225151 & 0.01$^{+0.007}_{-0.003}$ & 0.01$^{+0.007}_{-0.003}$ & 1,2,3,4,5,6,7,8,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4 & \nodata & \nodata\\
HIP 5158 b & 165722603 & 0.009$^{+0.002}_{-0.002}$ & 0.0007$^{+0.0002}_{-0.0001}$ & 3 & 1 & \nodata & \nodata\\
HD 210277 b & 50227884 & 0.0094$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 147379 b & 230073581 & 0.009$^{+0.001}_{-0.001}$ & 0.009$^{+0.001}_{-0.001}$ & \nodata & \nodata & 1,3,4,5,6,7,8,9,10,11,13 & 4,4,4,4,4,4,4,4,4,4,4\\
HIP 14810 c & 113810736 & 0.0093$^{+0.0006}_{-0.0006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
Kepler-56 d & 138430034 & 0.0092$^{+0.0005}_{-0.0005}$ & 0.00025$^{+0.00001}_{-0.00001}$ & \nodata & \nodata & 1 & 3\\
HIP 109384 b & 165454978 & 0.009$^{+0.001}_{-0.001}$ & 0.0015$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 3,4,5 & 3,3,3\\
HD 218566 b & 278952345 & 0.009$^{+0.002}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 141399 c & 419015728 & 0.009$^{+0.0007}_{-0.0007}$ & 0.0024$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 10,11 & 3,3\\
kap CrB b & 334753043 & 0.009$^{+0.0002}_{-0.0002}$ & 0.000193$^{+0.000005}_{-0.000005}$ & \nodata & \nodata & 11 & 2\\
HD 4113 b & 118586897 & 0.009$^{+0.001}_{-0.001}$ & 0.00046$^{+0.00007}_{-0.00006}$ & 2 & 2 & \nodata & \nodata\\
HD 92788 b & 265373654 & 0.009$^{+0.0003}_{-0.0003}$ & 0.00074$^{+0.00002}_{-0.00002}$ & 9 & 1 & \nodata & \nodata\\
BD-06 1339 c & 280304863 & 0.009$^{+0.002}_{-0.002}$ & 0.0019$^{+0.0005}_{-0.0004}$ & 6 & 1 & \nodata & \nodata\\
HD 33564 b & 142103211 & 0.009$^{+0.004}_{-0.004}$ & 0.0012$^{+0.0006}_{-0.0006}$ & \nodata & \nodata & 5,6 & 3,3\\
HD 27442 b & 198079199 & 0.0088$^{+0.0009}_{-0.0009}$ & 0.0033$^{+0.0004}_{-0.0003}$ & 2,3,4,5,8,12 & 4,3,3,4,4,4 & \nodata & \nodata\\
HD 41004 A b & 405228516 & 0.009$^{+0.01}_{-0.006}$ & 0.0007$^{+0.001}_{-0.0005}$ & 5,6,7 & 3,3,3 & \nodata & \nodata\\
HD 5319 c & 344627954 & 0.0087$^{+0.0006}_{-0.0006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 159868 c & 362661163 & 0.0087$^{+0.0005}_{-0.0004}$ & 0.00067$^{+0.00004}_{-0.00003}$ & 12 & 1 & \nodata & \nodata\\
HD 20794 e & 471011796 & 0.009$^{+0.002}_{-0.001}$ & 0.0031$^{+0.0007}_{-0.0005}$ & 3,4 & 3,3 & \nodata & \nodata\\
61 Vir d & 95359428 & 0.0085$^{+0.001}_{-0.0008}$ & 0.0019$^{+0.0002}_{-0.0002}$ & 10 & 1 & \nodata & \nodata\\
HD 65216 c & 408047845 & 0.0083$^{+0.0006}_{-0.0005}$ & 0.0083$^{+0.0006}_{-0.0005}$ & 1,2,3,4,5,7,8,9,10,11,12,13 & 4,4,4,4,4,4,4,3,4,4,4,4 & \nodata & \nodata\\
BD+14 4559 b & 95359428 & 0.0083$^{+0.0008}_{-0.0007}$ & 0.00083$^{+0.00008}_{-0.00007}$ & \nodata & \nodata & 1 & 1\\
HD 100777 b & 458582777 & 0.0082$^{+0.0004}_{-0.0004}$ & 0.00058$^{+0.00003}_{-0.00003}$ & 9 & 1 & \nodata & \nodata\\
HD 9446 c & 18277196 & 0.008$^{+0.004}_{-0.004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 142245 b & 68165288 & 0.0079$^{+0.0004}_{-0.0004}$ & 0.000165$^{+0.000008}_{-0.000008}$ & \nodata & \nodata & 11 & 2\\
HD 137388 A b & 236339228 & 0.008$^{+0.002}_{-0.001}$ & 0.0013$^{+0.0003}_{-0.0002}$ & 12,13 & 3,3 & \nodata & \nodata\\
HD 175167 b & 48917782 & 0.008$^{+0.002}_{-0.001}$ & 0.00016$^{+0.00004}_{-0.00003}$ & 13 & 2 & \nodata & \nodata\\
HIP 67851 c & 111947706 & 0.0078$^{+0.001}_{-0.0008}$ & 0.0001$^{+0.00001}_{-0.00001}$ & 11 & 1 & \nodata & \nodata\\
HD 60532 c & 456871289 & 0.0078$^{+0.0005}_{-0.0004}$ & 0.00035$^{+0.00002}_{-0.00002}$ & 7 & 2 & \nodata & \nodata\\
ups And c & 189576919 & 0.008$^{+0.004}_{-0.004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 220842 b & 165454978 & 0.0078$^{+0.0004}_{-0.0003}$ & 0.00193$^{+0.00009}_{-0.00008}$ & \nodata & \nodata & 3,4 & 3,2\\
HD 45364 b & 117768715 & 0.0078$^{+0.001}_{-0.0008}$ & 0.0018$^{+0.0002}_{-0.0002}$ & 6,7 & 3,3 & \nodata & \nodata\\
HD 153950 b & 21897561 & 0.0077$^{+0.0004}_{-0.0003}$ & 0.00042$^{+0.00002}_{-0.00002}$ & 12 & 1 & \nodata & \nodata\\
HD 125612 b & 349606708 & 0.0075$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 164604 b & 302317605 & 0.007$^{+0.007}_{-0.006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
7 CMa b & 356478817 & 0.0074$^{+0.0008}_{-0.0007}$ & 0.00025$^{+0.00003}_{-0.00002}$ & 6 & 2 & \nodata & \nodata\\
HD 113337 b & 243194645 & 0.007$^{+0.001}_{-0.001}$ & 0.0012$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 8,9 & 3,3\\
HD 159243 c & 362661163 & 0.0074$^{+0.0006}_{-0.0006}$ & 0.0008$^{+0.00007}_{-0.00006}$ & \nodata & \nodata & 12 & 1\\
Wolf 1061 d & 413948621 & 0.007$^{+0.002}_{-0.001}$ & 0.0009$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 12 & 1\\
HR 810 b & 166853853 & 0.007$^{+0.001}_{-0.001}$ & 0.0013$^{+0.0002}_{-0.0002}$ & 2,3 & 3,3 & \nodata & \nodata\\
HD 75898 b & 46310554 & 0.0073$^{+0.0005}_{-0.0005}$ & 0.00047$^{+0.00003}_{-0.00003}$ & \nodata & \nodata & 7 & 1\\
HD 1666 b & 211439561 & 0.007$^{+0.002}_{-0.002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 11506 c & 266680498 & 0.0072$^{+0.0004}_{-0.0003}$ & 0.00087$^{+0.00005}_{-0.00004}$ & 3 & 1 & \nodata & \nodata\\
HD 4732 c & 268397995 & 0.0071$^{+0.001}_{-0.0008}$ & 0.00007$^{+0.000009}_{-0.000008}$ & 3 & 1 & \nodata & \nodata\\
55 Cnc f & 332064670 & 0.007$^{+0.0008}_{-0.0006}$ & 0.00072$^{+0.00008}_{-0.00006}$ & \nodata & \nodata & 7 & 1\\
HD 38801 b & 374859347 & 0.007$^{+0.0002}_{-0.0002}$ & 0.000272$^{+0.000009}_{-0.000009}$ & 6 & 2 & \nodata & \nodata\\
HD 155358 c & 75673519 & 0.007$^{+0.0007}_{-0.0004}$ & 0.00048$^{+0.00005}_{-0.00003}$ & \nodata & \nodata & 12 & 3\\
HD 213240 b & 154487334 & 0.0069$^{+0.0002}_{-0.0002}$ & 0.000211$^{+0.000006}_{-0.000006}$ & 1 & 2 & \nodata & \nodata\\
HD 142 b & 389757979 & 0.0069$^{+0.0006}_{-0.0005}$ & 0.00053$^{+0.00004}_{-0.00004}$ & 2 & 2 & \nodata & \nodata\\
HD 156411 b & 348652846 & 0.0069$^{+0.0008}_{-0.0006}$ & 0.00022$^{+0.00003}_{-0.00002}$ & 12 & 1 & \nodata & \nodata\\
GJ 3021 b & 77897915 & 0.007$^{+0.003}_{-0.003}$ & 0.0014$^{+0.0006}_{-0.0006}$ & 1 & 3 & \nodata & \nodata\\
eps Eri b & 367912480 & 0.007$^{+0.007}_{-0.006}$ & 0.00007$^{+0.00007}_{-0.00007}$ & 4 & 1 & \nodata & \nodata\\
HIP 97233 b & 251662732 & 0.0068$^{+0.0007}_{-0.0007}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 45350 b & 144132551 & 0.007$^{+0.003}_{-0.003}$ & 0.00019$^{+0.00009}_{-0.00009}$ & \nodata & \nodata & 6 & 1\\
HIP 79431 b & 49324530 & 0.007$^{+0.003}_{-0.003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
Kepler-424 c & 437034879 & 0.0067$^{+0.0009}_{-0.0008}$ & 0.0016$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & 1,2 & 3,3\\
BD-08 2823 c & 393702609 & 0.0067$^{+0.001}_{-0.0008}$ & 0.00076$^{+0.0001}_{-0.00009}$ & 8 & 1 & \nodata & \nodata\\
HD 183263 b & 469943599 & 0.0066$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
CoRoT-20 c & 234825296 & 0.007$^{+0.006}_{-0.006}$ & 0.0001$^{+0.0001}_{-0.0001}$ & 6 & 1 & \nodata & \nodata\\
BD-17 63 b & 33355302 & 0.0065$^{+0.0004}_{-0.0003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 3293 c & 267399515 & 0.0065$^{+0.001}_{-0.0007}$ & 0.0014$^{+0.0002}_{-0.0002}$ & 5 & 2 & \nodata & \nodata\\
HD 164509 b & 16465196 & 0.006$^{+0.002}_{-0.001}$ & 0.0006$^{+0.0002}_{-0.0001}$ & \nodata & \nodata & 13 & 1\\
HD 23127 b & 311924816 & 0.0063$^{+0.0009}_{-0.0007}$ & 0.00042$^{+0.00006}_{-0.00005}$ & 2,3,4 & 3,3,3 & \nodata & \nodata\\
HD 160691 e & 382764222 & 0.0063$^{+0.0008}_{-0.0007}$ & 0.00055$^{+0.00007}_{-0.00006}$ & 12 & 1 & \nodata & \nodata\\
HD 205739 b & 270501383 & 0.0063$^{+0.0006}_{-0.0005}$ & 0.00061$^{+0.00005}_{-0.00005}$ & 1 & 1 & \nodata & \nodata\\
HD 67087 b & 307624961 & 0.006$^{+0.001}_{-0.001}$ & 0.0005$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 7 & 1\\
HD 63765 b & 471011546 & 0.0062$^{+0.0004}_{-0.0004}$ & 0.00141$^{+0.00009}_{-0.00008}$ & 7,8,9 & 3,3,3 & \nodata & \nodata\\
HD 215497 c & 47526465 & 0.0062$^{+0.0009}_{-0.0008}$ & 0.0003$^{+0.00004}_{-0.00004}$ & 1 & 2 & \nodata & \nodata\\
HD 108341 b & 154549250 & 0.006$^{+0.006}_{-0.002}$ & 0.0003$^{+0.0003}_{-0.00009}$ & 11,12 & 3,3 & \nodata & \nodata\\
HIP 109600 b & 251866143 & 0.0062$^{+0.0003}_{-0.0003}$ & 0.00072$^{+0.00004}_{-0.00004}$ & \nodata & \nodata & 2 & 2\\
HD 129445 b & 309808219 & 0.006$^{+0.007}_{-0.006}$ & 0.00009$^{+0.0001}_{-0.00008}$ & 12 & 2 & \nodata & \nodata\\
tau Cet f & 439403362 & 0.006$^{+0.006}_{-0.006}$ & 0.0003$^{+0.0003}_{-0.0003}$ & 3 & 1 & \nodata & \nodata\\
HD 219077 b & 354326161 & 0.0061$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 19994 b & 301051051 & 0.006$^{+0.006}_{-0.006}$ & 0.0004$^{+0.0003}_{-0.0003}$ & 4 & 1 & \nodata & \nodata\\
GJ 3323 c & 318686860 & 0.006$^{+0.002}_{-0.002}$ & 0.004$^{+0.002}_{-0.001}$ & 5 & 1 & \nodata & \nodata\\
HD 108874 b & 429301734 & 0.006$^{+0.0002}_{-0.0002}$ & 0.00041$^{+0.00002}_{-0.00002}$ & \nodata & \nodata & 9 & 1\\
HD 141937 b & 290493086 & 0.006$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
WASP-47 c & 397288169 & 0.0059$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 73526 c & 302368715 & 0.0059$^{+0.0003}_{-0.0003}$ & 0.00084$^{+0.00004}_{-0.00004}$ & 8,9 & 3,3 & \nodata & \nodata\\
HD 45364 c & 1713457 & 0.0058$^{+0.0007}_{-0.0006}$ & 0.00091$^{+0.0001}_{-0.00009}$ & 6,7 & 3,3 & \nodata & \nodata\\
HD 65216 b & 340697083 & 0.0058$^{+0.0007}_{-0.0006}$ & 0.0031$^{+0.0004}_{-0.0003}$ & 1,2,3,4,5,7,8,9,10,11,12,13 & 4,4,4,4,4,4,4,3,4,4,4,4 & \nodata & \nodata\\
HAT-P-44 c & 168699373 & 0.0057$^{+0.001}_{-0.0008}$ & 0.00035$^{+0.00007}_{-0.00005}$ & \nodata & \nodata & 9,10 & 3,3\\
HD 48265 b & 255781806 & 0.0056$^{+0.0005}_{-0.0004}$ & 0.00058$^{+0.00005}_{-0.00004}$ & 6,7,8 & 3,3,3 & \nodata & \nodata\\
HD 219828 c & 95361265 & 0.0056$^{+0.0006}_{-0.0005}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 181720 b & 144068704 & 0.0055$^{+0.0006}_{-0.0005}$ & 0.00016$^{+0.00002}_{-0.00001}$ & 13 & 1 & \nodata & \nodata\\
HD 145934 b & 413853880 & 0.0055$^{+0.0006}_{-0.0005}$ & 0.000054$^{+0.000006}_{-0.000005}$ & \nodata & \nodata & 11 & 2\\
HD 28185 b & 452910671 & 0.0055$^{+0.0002}_{-0.0002}$ & 0.00039$^{+0.00002}_{-0.00002}$ & 5 & 2 & \nodata & \nodata\\
HD 1605 c & 122555698 & 0.0054$^{+0.0002}_{-0.0002}$ & 0.00007$^{+0.000003}_{-0.000003}$ & \nodata & \nodata & 3 & 1\\
HD 196885 b & 282257777 & 0.0053$^{+0.0007}_{-0.0006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 187085 b & 300081980 & 0.0053$^{+0.0006}_{-0.0005}$ & 0.00015$^{+0.00002}_{-0.00001}$ & 13 & 1 & \nodata & \nodata\\
HD 128311 b & 189694184 & 0.0052$^{+0.0002}_{-0.0002}$ & 0.00031$^{+0.00001}_{-0.00001}$ & \nodata & \nodata & 11 & 1\\
HD 81040 b & 85998162 & 0.0052$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 3138 d & 471012347 & 0.005$^{+0.002}_{-0.001}$ & 0.0005$^{+0.0002}_{-0.0001}$ & 3 & 1 & \nodata & \nodata\\
HD 132406 b & 61397572 & 0.0052$^{+0.0009}_{-0.0007}$ & 0.00029$^{+0.00005}_{-0.00004}$ & \nodata & \nodata & 9,10 & 3,3\\
HD 99109 b & 156942082 & 0.0051$^{+0.0008}_{-0.0006}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 224538 b & 280803137 & 0.0051$^{+0.0003}_{-0.0003}$ & 0.00023$^{+0.00001}_{-0.00001}$ & 1,2 & 2,3 & \nodata & \nodata\\
HD 221287 b & 231716612 & 0.005$^{+0.001}_{-0.001}$ & 0.0003$^{+0.00007}_{-0.00006}$ & 1 & 2 & \nodata & \nodata\\
Kapteyn c & 142350121 & 0.005$^{+0.001}_{-0.0009}$ & 0.0033$^{+0.0008}_{-0.0006}$ & 4,5,6 & 3,3,3 & \nodata & \nodata\\
HD 192310 c & 195382102 & 0.0049$^{+0.001}_{-0.0008}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 17674 b & 77490014 & 0.0049$^{+0.0004}_{-0.0004}$ & 0.00021$^{+0.00002}_{-0.00002}$ & \nodata & \nodata & 4 & 1\\
HD 131664 b & 407090552 & 0.0048$^{+0.0002}_{-0.0002}$ & 0.000067$^{+0.000002}_{-0.000002}$ & 12 & 2 & \nodata & \nodata\\
HD 126614 b & 258186667 & 0.0048$^{+0.001}_{-0.0007}$ & 0.0001$^{+0.00002}_{-0.00002}$ & \nodata & \nodata & 11 & 1\\
HD 82943 b & 348964243 & 0.005$^{+0.002}_{-0.002}$ & 0.0003$^{+0.0001}_{-0.0001}$ & 8 & 1 & \nodata & \nodata\\
HD 34445 b & 284907742 & 0.0046$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 188015 b & 11499710 & 0.005$^{+0.002}_{-0.002}$ & 0.0003$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & 1 & 2\\
HD 73534 b & 180661948 & 0.0046$^{+0.0004}_{-0.0004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 133131 A b & 440955225 & 0.0046$^{+0.0004}_{-0.0004}$ & 0.00019$^{+0.00002}_{-0.00001}$ & 11 & 1 & \nodata & \nodata\\
HD 7199 b & 52121796 & 0.0045$^{+0.001}_{-0.0008}$ & 0.0004$^{+0.0001}_{-0.00007}$ & 1,2 & 3,3 & \nodata & \nodata\\
Kepler-454 c & 121276638 & 0.0045$^{+0.0005}_{-0.0005}$ & 0.00047$^{+0.00006}_{-0.00005}$ & \nodata & \nodata & 1,13 & 3,3\\
HD 50554 b & 80224448 & 0.0045$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 876 e & 231836962 & 0.004$^{+0.002}_{-0.002}$ & 0.001$^{+0.0004}_{-0.0004}$ & 2 & 1 & \nodata & \nodata\\
HD 217786 b & 248048656 & 0.0045$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 85390 b & 80535228 & 0.0045$^{+0.001}_{-0.0008}$ & 0.00031$^{+0.00008}_{-0.00005}$ & 9,10 & 3,3 & \nodata & \nodata\\
HD 114729 b & 82605074 & 0.0045$^{+0.0003}_{-0.0003}$ & 0.000108$^{+0.000008}_{-0.000007}$ & 10 & 1 & \nodata & \nodata\\
HD 148156 b & 159511543 & 0.0044$^{+0.0006}_{-0.0006}$ & 0.00012$^{+0.00002}_{-0.00002}$ & 12 & 1 & \nodata & \nodata\\
HIP 57274 d & 5078530 & 0.0044$^{+0.0006}_{-0.0005}$ & 0.00027$^{+0.00004}_{-0.00003}$ & \nodata & \nodata & 9 & 1\\
WASP-41 c & 102987456 & 0.0043$^{+0.0003}_{-0.0003}$ & 0.00028$^{+0.00002}_{-0.00002}$ & 10 & 1 & \nodata & \nodata\\
HD 34445 f & 388804061 & 0.0043$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
Kepler-68 d & 437038987 & 0.0043$^{+0.0003}_{-0.0003}$ & 0.00056$^{+0.00004}_{-0.00004}$ & \nodata & \nodata & 1,2,13 & 3,3,3\\
HD 219415 b & 323819453 & 0.0043$^{+0.0009}_{-0.0008}$ & 0.00011$^{+0.00002}_{-0.00002}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 22781 b & 101166776 & 0.0043$^{+0.0002}_{-0.0002}$ & 0.00022$^{+0.00001}_{-0.00001}$ & \nodata & \nodata & 5 & 1\\
HD 190647 b & 351534793 & 0.0043$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 114783 b & 180030300 & 0.0043$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 159868 b & 362661163 & 0.0043$^{+0.0001}_{-0.0001}$ & 0.000098$^{+0.000003}_{-0.000003}$ & 12 & 1 & \nodata & \nodata\\
HD 9174 b & 439501096 & 0.0042$^{+0.0004}_{-0.0003}$ & 0.000096$^{+0.000008}_{-0.000007}$ & 3 & 1 & \nodata & \nodata\\
HD 106252 b & 371621400 & 0.0042$^{+0.0001}_{-0.0001}$ & 0.000073$^{+0.000003}_{-0.000002}$ & \nodata & \nodata & 9 & 1\\
HD 564 b & 382625142 & 0.0041$^{+0.0003}_{-0.0003}$ & 0.00023$^{+0.00002}_{-0.00002}$ & 2 & 2 & \nodata & \nodata\\
HD 160691 b & 367987991 & 0.0041$^{+0.0005}_{-0.0004}$ & 0.00017$^{+0.00002}_{-0.00002}$ & 12 & 1 & \nodata & \nodata\\
HD 13908 c & 12906712 & 0.0041$^{+0.0003}_{-0.0003}$ & 0.000119$^{+0.000008}_{-0.000008}$ & \nodata & \nodata & 5 & 2\\
HD 196067 b & 327303574 & 0.004$^{+0.003}_{-0.001}$ & 0.000031$^{+0.00002}_{-0.000007}$ & 13 & 3 & \nodata & \nodata\\
HD 165155 b & 408229533 & 0.0041$^{+0.0005}_{-0.0005}$ & 0.00026$^{+0.00003}_{-0.00003}$ & 13 & 1 & \nodata & \nodata\\
HD 43197 b & 37660988 & 0.004$^{+0.001}_{-0.0006}$ & 0.00033$^{+0.0001}_{-0.00005}$ & 6 & 2 & \nodata & \nodata\\
HD 216437 b & 394125166 & 0.004$^{+0.002}_{-0.002}$ & 0.00009$^{+0.00005}_{-0.00004}$ & 1 & 3 & \nodata & \nodata\\
HD 111998 b & 21267079 & 0.004$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
GJ 667 C g & 233193964 & 0.0039$^{+0.001}_{-0.0008}$ & 0.00042$^{+0.0001}_{-0.00008}$ & 12 & 1 & \nodata & \nodata\\
HD 142022 A b & 69528586 & 0.004$^{+0.003}_{-0.001}$ & 0.00011$^{+0.00008}_{-0.00003}$ & 12,13 & 3,3 & \nodata & \nodata\\
GJ 163 d & 219221189 & 0.0039$^{+0.0007}_{-0.0006}$ & 0.00052$^{+0.0001}_{-0.00008}$ & 3,4,5 & 3,3,3 & \nodata & \nodata\\
HD 106515 A b & 371621238 & 0.0039$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 23079 b & 206402844 & 0.0038$^{+0.0002}_{-0.0002}$ & 0.00028$^{+0.00001}_{-0.00001}$ & 3,4 & 3,3 & \nodata & \nodata\\
HD 75784 b & 379949822 & 0.004$^{+0.003}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 23596 b & 201266092 & 0.0038$^{+0.0001}_{-0.0001}$ & 0.000065$^{+0.000002}_{-0.000002}$ & \nodata & \nodata & 5 & 1\\
HD 106270 b & 286896213 & 0.0037$^{+0.0005}_{-0.0004}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 216435 b & 156067565 & 0.004$^{+0.002}_{-0.002}$ & 0.00008$^{+0.00004}_{-0.00004}$ & 1 & 2 & \nodata & \nodata\\
HD 196050 b & 49845357 & 0.0037$^{+0.0002}_{-0.0002}$ & 0.000073$^{+0.000005}_{-0.000004}$ & 13 & 2 & \nodata & \nodata\\
HD 221585 b & 245873777 & 0.0037$^{+0.0004}_{-0.0003}$ & 0.000085$^{+0.000009}_{-0.000008}$ & \nodata & \nodata & 4 & 3\\
HD 10180 g & 397558558 & 0.0037$^{+0.0009}_{-0.0006}$ & 0.00033$^{+0.00008}_{-0.00005}$ & 1,2 & 3,3 & \nodata & \nodata\\
HD 66428 b & 452867458 & 0.0035$^{+0.0002}_{-0.0002}$ & 0.000048$^{+0.000003}_{-0.000003}$ & 7 & 1 & \nodata & \nodata\\
HD 147513 b & 255930614 & 0.003$^{+0.002}_{-0.002}$ & 0.00018$^{+0.00009}_{-0.00009}$ & 12 & 1 & \nodata & \nodata\\
HD 11506 b & 266680498 & 0.0035$^{+0.0006}_{-0.0005}$ & 0.000067$^{+0.00001}_{-0.000009}$ & 3 & 1 & \nodata & \nodata\\
HD 168443 c & 320362897 & 0.0033$^{+0.0001}_{-0.0001}$ & 0.000051$^{+0.000002}_{-0.000002}$ & \nodata & \nodata & 13 & 1\\
HD 42012 b & 97724459 & 0.0033$^{+0.0003}_{-0.0003}$ & 0.0001$^{+0.00001}_{-0.00001}$ & \nodata & \nodata & 6 & 1\\
HD 163607 c & 16465196 & 0.0033$^{+0.0004}_{-0.0003}$ & 0.00088$^{+0.0001}_{-0.00008}$ & \nodata & \nodata & 1,2,3,4,5,6,7,8,9,10,11,12,13 & 4,4,4,4,4,4,4,4,4,4,4,4,4\\
HD 170469 b & 467966544 & 0.0032$^{+0.0003}_{-0.0003}$ & 0.000075$^{+0.000008}_{-0.000007}$ & \nodata & \nodata & 13 & 2\\
Kepler-97 c & 399951991 & 0.0031$^{+0.0004}_{-0.0003}$ & 0.00022$^{+0.00002}_{-0.00002}$ & \nodata & \nodata & 1,13 & 3,3\\
HD 28254 b & 219256496 & 0.0031$^{+0.0004}_{-0.0003}$ & 0.00023$^{+0.00003}_{-0.00002}$ & 3,4,5 & 3,3,3 & \nodata & \nodata\\
HD 4208 b & 43400838 & 0.0031$^{+0.0002}_{-0.0002}$ & 0.000101$^{+0.000005}_{-0.000005}$ & 3 & 1 & \nodata & \nodata\\
HD 214823 b & 471011442 & 0.0031$^{+0.0004}_{-0.0004}$ & 0.000045$^{+0.000006}_{-0.000006}$ & \nodata & \nodata & 2 & 2\\
HD 114386 b & 288474555 & 0.0031$^{+0.0002}_{-0.0002}$ & 0.000089$^{+0.000005}_{-0.000005}$ & 10 & 1 & \nodata & \nodata\\
HD 171238 b & 265052133 & 0.0031$^{+0.0004}_{-0.0003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 207832 c & 53895723 & 0.0031$^{+0.001}_{-0.0004}$ & 0.00007$^{+0.00002}_{-0.00001}$ & 1 & 1 & \nodata & \nodata\\
GJ 676 A b & 139754153 & 0.0031$^{+0.0003}_{-0.0003}$ & 0.000079$^{+0.000008}_{-0.000008}$ & 12 & 1 & \nodata & \nodata\\
HD 111232 b & 124306858 & 0.00299$^{+0.0001}_{-0.00009}$ & 0.000071$^{+0.000002}_{-0.000002}$ & 11 & 3 & \nodata & \nodata\\
KELT-6 c & 232620788 & 0.003$^{+0.0003}_{-0.0002}$ & 0.000063$^{+0.000006}_{-0.000005}$ & \nodata & \nodata & 9 & 2\\
47 UMa b & 332064670 & 0.003$^{+0.001}_{-0.001}$ & 0.00007$^{+0.00003}_{-0.00003}$ & \nodata & \nodata & 8 & 2\\
HD 141399 d & 283722336 & 0.0029$^{+0.0002}_{-0.0002}$ & 0.00015$^{+0.00001}_{-0.00001}$ & \nodata & \nodata & 10,11 & 3,3\\
HD 181433 c & 326096771 & 0.0029$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 8535 b & 41862035 & 0.0029$^{+0.0003}_{-0.0002}$ & 0.000117$^{+0.00001}_{-0.000009}$ & 2,3 & 2,2 & \nodata & \nodata\\
HD 11964 b & 118268680 & 0.0028$^{+0.0003}_{-0.0003}$ & 0.000039$^{+0.000005}_{-0.000004}$ & 3 & 1 & \nodata & \nodata\\
HD 86264 b & 61125572 & 0.0028$^{+0.001}_{-0.0005}$ & 0.000051$^{+0.00002}_{-0.000009}$ & 8 & 1 & \nodata & \nodata\\
HD 113538 b & 138172859 & 0.0028$^{+0.0003}_{-0.0003}$ & 0.00011$^{+0.00001}_{-0.00001}$ & 11 & 2 & \nodata & \nodata\\
HD 8673 b & 169248301 & 0.0028$^{+0.0003}_{-0.0003}$ & 0.000046$^{+0.000005}_{-0.000005}$ & \nodata & \nodata & 4 & 1\\
Pr0211 c & 123309556 & 0.003$^{+0.004}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 47186 c & 268565917 & 0.0027$^{+0.0005}_{-0.0004}$ & 0.00011$^{+0.00002}_{-0.00001}$ & 6,7 & 2,2 & \nodata & \nodata\\
HD 10647 b & 252803484 & 0.0027$^{+0.0002}_{-0.0002}$ & 0.00015$^{+0.00001}_{-0.00001}$ & 2,3 & 3,3 & \nodata & \nodata\\
psi 1 Dra B b & 441804565 & 0.0027$^{+0.0004}_{-0.0004}$ & 0.00025$^{+0.00004}_{-0.00004}$ & \nodata & \nodata & 1,2,4,5,6,7,8,9,10,11,12 & 4,4,4,4,4,4,4,4,4,4,4\\
14 Her b & 333225860 & 0.00263$^{+0.00009}_{-0.00009}$ & 0.00008$^{+0.000003}_{-0.000003}$ & \nodata & \nodata & 10,11 & 3,3\\
HD 38529 c & 200093173 & 0.003$^{+0.002}_{-0.002}$ & 0.00003$^{+0.00003}_{-0.00003}$ & 6 & 1 & \nodata & \nodata\\
GJ 649 b & 36853511 & 0.0026$^{+0.0004}_{-0.0003}$ & 0.00012$^{+0.00002}_{-0.00001}$ & \nodata & \nodata & 12 & 2\\
Kepler-94 c & 175290574 & 0.0025$^{+0.0001}_{-0.0001}$ & 0.000167$^{+0.000008}_{-0.000008}$ & \nodata & \nodata & 1,13 & 3,3\\
Kepler-48 e & 171882123 & 0.0025$^{+0.0001}_{-0.0001}$ & 0.00007$^{+0.000004}_{-0.000004}$ & \nodata & \nodata & 1 & 3\\
HD 204941 b & 99837626 & 0.0025$^{+0.0004}_{-0.0003}$ & 0.00004$^{+0.000006}_{-0.000005}$ & 1 & 1 & \nodata & \nodata\\
HD 87883 b & 193032655 & 0.0025$^{+0.0009}_{-0.0005}$ & 0.000025$^{+0.000009}_{-0.000005}$ & \nodata & \nodata & 8 & 1\\
HD 29021 b & 458350670 & 0.0025$^{+0.0003}_{-0.0003}$ & 0.00005$^{+0.000005}_{-0.000005}$ & \nodata & \nodata & 5 & 2\\
HD 164922 b & 18097734 & 0.0025$^{+0.0003}_{-0.0002}$ & 0.00012$^{+0.00001}_{-0.00001}$ & \nodata & \nodata & 12,13 & 2,2\\
HD 128311 c & 267365022 & 0.00251$^{+0.00009}_{-0.00009}$ & 0.000073$^{+0.000003}_{-0.000003}$ & \nodata & \nodata & 11 & 1\\
HIP 14810 d & 113810736 & 0.0025$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 10697 b & 456905162 & 0.00245$^{+0.00007}_{-0.00006}$ & 0.000062$^{+0.000002}_{-0.000002}$ & \nodata & \nodata & 4 & 1\\
HD 147018 c & 198562505 & 0.0024$^{+0.0001}_{-0.0001}$ & 0.000065$^{+0.000004}_{-0.000003}$ & 12 & 2 & \nodata & \nodata\\
HD 68402 b & 272546396 & 0.0024$^{+0.0002}_{-0.0002}$ & 0.00054$^{+0.00004}_{-0.00004}$ & 2,3,6,7,9,10,11,12,13 & 4,4,4,4,4,4,3,4,4 & \nodata & \nodata\\
HD 108874 c & 144289338 & 0.0024$^{+0.0001}_{-0.0001}$ & 0.00004$^{+0.000002}_{-0.000002}$ & \nodata & \nodata & 9 & 1\\
ups And d & 283722336 & 0.002$^{+0.001}_{-0.001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 132563 b & 471011913 & 0.0024$^{+0.0004}_{-0.0003}$ & 0.000042$^{+0.000007}_{-0.000005}$ & \nodata & \nodata & 10 & 3\\
HD 197037 b & 333314269 & 0.0024$^{+0.0004}_{-0.0004}$ & 0.00013$^{+0.00002}_{-0.00002}$ & \nodata & \nodata & 1,2 & 3,3\\
HD 204313 b & 99734092 & 0.0024$^{+0.0002}_{-0.0001}$ & 0.000034$^{+0.000002}_{-0.000002}$ & 1 & 1 & \nodata & \nodata\\
GJ 317 b & 219221189 & 0.0024$^{+0.0003}_{-0.0003}$ & 0.00009$^{+0.00001}_{-0.00001}$ & 8 & 2 & \nodata & \nodata\\
GJ 1148 c & 471011718 & 0.002$^{+0.001}_{-0.001}$ & 0.00012$^{+0.00005}_{-0.00005}$ & \nodata & \nodata & 8 & 2\\
HD 12661 c & 118268680 & 0.00225$^{+0.00007}_{-0.00007}$ & 0.000036$^{+0.000001}_{-0.000001}$ & \nodata & \nodata & 4 & 1\\
HD 143361 b & 272783172 & 0.0022$^{+0.0002}_{-0.0002}$ & 0.000058$^{+0.000005}_{-0.000005}$ & 12 & 1 & \nodata & \nodata\\
HD 133131 A c & 53304943 & 0.0022$^{+0.002}_{-0.0008}$ & 0.000017$^{+0.00001}_{-0.000006}$ & 11 & 1 & \nodata & \nodata\\
HD 89307 b & 345078350 & 0.0022$^{+0.0002}_{-0.0001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 133131 B b & 101145648 & 0.0021$^{+0.0004}_{-0.0003}$ & 0.00001$^{+0.000002}_{-0.000001}$ & 11 & 1 & \nodata & \nodata\\
HD 190360 b & 105999792 & 0.00214$^{+0.00009}_{-0.00009}$ & 0.0000199$^{+0.0000008}_{-0.0000008}$ & \nodata & \nodata & 1 & 2\\
HD 222155 b & 26370518 & 0.0021$^{+0.0008}_{-0.0005}$ & 0.000014$^{+0.000005}_{-0.000003}$ & \nodata & \nodata & 3 & 2\\
HD 73267 b & 121284864 & 0.002$^{+0.001}_{-0.001}$ & 0.00005$^{+0.00002}_{-0.00002}$ & 8 & 2 & \nodata & \nodata\\
HD 191806 b & 243085377 & 0.0021$^{+0.0002}_{-0.0002}$ & 0.000071$^{+0.000005}_{-0.000005}$ & \nodata & \nodata & 1,2 & 3,3\\
HD 30669 b & 607907 & 0.0021$^{+0.0005}_{-0.0003}$ & 0.000034$^{+0.000007}_{-0.000005}$ & 5 & 2 & \nodata & \nodata\\
HD 154857 c & 248320609 & 0.0021$^{+0.0001}_{-0.0001}$ & 0.0000164$^{+0.0000008}_{-0.0000008}$ & 12 & 2 & \nodata & \nodata\\
HD 25171 b & 237933846 & 0.0021$^{+0.0002}_{-0.0002}$ & 0.00027$^{+0.00003}_{-0.00002}$ & 1,2,3,4,7,8,10,11,13 & 4,3,4,4,4,4,4,4,4 & \nodata & \nodata\\
HD 169830 c & 157951225 & 0.002$^{+0.001}_{-0.001}$ & 0.00003$^{+0.00001}_{-0.00001}$ & 13 & 1 & \nodata & \nodata\\
HD 39091 b & 261136679 & 0.002$^{+0.0002}_{-0.0002}$ & 0.00015$^{+0.00002}_{-0.00002}$ & 1,4,8,11,12,13 & 4,4,4,4,3,3 & \nodata & \nodata\\
Kepler-93 c & 137151335 & 0.002$^{+0.0002}_{-0.0002}$ & 0.000073$^{+0.000007}_{-0.000006}$ & \nodata & \nodata & 1,13 & 3,3\\
HD 72659 b & 183356952 & 0.00198$^{+0.00009}_{-0.00009}$ & 0.0000146$^{+0.0000007}_{-0.0000006}$ & 7 & 1 & \nodata & \nodata\\
HAT-P-11 c & 28230919 & 0.0019$^{+0.0002}_{-0.0002}$ & 0.00003$^{+0.000004}_{-0.000003}$ & \nodata & \nodata & 1,2 & 3,3\\
HD 30177 b & 220408612 & 0.0019$^{+0.0001}_{-0.0001}$ & 0.00018$^{+0.00001}_{-0.00001}$ & 2,3,4,5,6,8,9,10,12,13 & 4,4,3,4,4,4,4,4,4,4 & \nodata & \nodata\\
HD 86226 b & 8154501 & 0.0019$^{+0.0003}_{-0.0002}$ & 0.00003$^{+0.000004}_{-0.000003}$ & 9 & 2 & \nodata & \nodata\\
HD 70573 b & 180661948 & 0.0018$^{+0.0003}_{-0.0002}$ & 0.000059$^{+0.000008}_{-0.000008}$ & 7 & 1 & \nodata & \nodata\\
HD 202206 c & 24294415 & 0.0018$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 220689 b & 9156146 & 0.0018$^{+0.0003}_{-0.0002}$ & 0.000022$^{+0.000003}_{-0.000003}$ & 2 & 1 & \nodata & \nodata\\
HD 117207 b & 347909637 & 0.00178$^{+0.0001}_{-0.00009}$ & 0.0000185$^{+0.000001}_{-0.0000009}$ & 11 & 1 & \nodata & \nodata\\
47 UMa c & 233721425 & 0.0018$^{+0.0008}_{-0.0008}$ & 0.00002$^{+0.000009}_{-0.000009}$ & \nodata & \nodata & 8 & 2\\
HD 79498 b & 37533318 & 0.0017$^{+0.0003}_{-0.0003}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 27631 b & 7652514 & 0.0017$^{+0.0008}_{-0.0008}$ & 0.00004$^{+0.00002}_{-0.00002}$ & 4,5 & 3,3 & \nodata & \nodata\\
HD 70642 b & 307624961 & 0.00172$^{+0.00009}_{-0.00008}$ & 0.000022$^{+0.000001}_{-0.000001}$ & 8 & 3 & \nodata & \nodata\\
HD 10180 h & 231836962 & 0.0017$^{+0.0002}_{-0.0002}$ & 0.000042$^{+0.000005}_{-0.000004}$ & 1,2 & 3,3 & \nodata & \nodata\\
HD 32963 b & 87989721 & 0.0016$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 114613 b & 24978373 & 0.0016$^{+0.0001}_{-0.0001}$ & 0.0000112$^{+0.0000009}_{-0.0000008}$ & 10 & 1 & \nodata & \nodata\\
HD 290327 b & 4205424 & 0.0016$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 6718 b & 455235218 & 0.0016$^{+0.0002}_{-0.0002}$ & 0.000017$^{+0.000002}_{-0.000002}$ & 3 & 1 & \nodata & \nodata\\
HD 67087 c & 73238215 & 0.0015$^{+0.0009}_{-0.0005}$ & 0.000017$^{+0.00001}_{-0.000005}$ & \nodata & \nodata & 7 & 1\\
HD 183263 c & 134245358 & 0.0014$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 152079 b & 232606278 & 0.0014$^{+0.0002}_{-0.0002}$ & 0.000013$^{+0.000002}_{-0.000002}$ & 12 & 1 & \nodata & \nodata\\
HD 181433 d & 317057430 & 0.0014$^{+0.0003}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 24040 b & 456863621 & 0.0014$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 166724 b & 281520119 & 0.0014$^{+0.0002}_{-0.0002}$ & 0.000007$^{+0.000001}_{-0.000001}$ & 13 & 1 & \nodata & \nodata\\
HD 141399 e & 283722336 & 0.0014$^{+0.0007}_{-0.0004}$ & 0.000015$^{+0.000008}_{-0.000004}$ & \nodata & \nodata & 10,11 & 3,3\\
GJ 849 b & 290543478 & 0.0013$^{+0.0002}_{-0.0002}$ & 0.000019$^{+0.000003}_{-0.000002}$ & \nodata & \nodata & 2 & 1\\
HD 219134 h & 116376059 & 0.00131$^{+0.00008}_{-0.00008}$ & 0.000032$^{+0.000002}_{-0.000002}$ & \nodata & \nodata & 3,4 & 3,3\\
HD 190984 b & 466222634 & 0.0013$^{+0.0007}_{-0.0006}$ & 0.000007$^{+0.000004}_{-0.000003}$ & 13 & 2 & \nodata & \nodata\\
BD-11 4672 b & 66914642 & 0.0013$^{+0.0001}_{-0.00009}$ & 0.000021$^{+0.000002}_{-0.000001}$ & \nodata & \nodata & 13 & 1\\
HD 37605 c & 374859347 & 0.0013$^{+0.00004}_{-0.00004}$ & 0.0000129$^{+0.0000004}_{-0.0000004}$ & 6 & 1 & \nodata & \nodata\\
Kepler-407 c & 283722336 & 0.0013$^{+0.0002}_{-0.0002}$ & 0.000035$^{+0.000005}_{-0.000004}$ & \nodata & \nodata & 1,2,13 & 3,3,3\\
HD 13931 b & 292851928 & 0.00126$^{+0.0001}_{-0.00009}$ & 0.0000081$^{+0.0000007}_{-0.0000006}$ & \nodata & \nodata & 4 & 1\\
HD 217107 c & 38271828 & 0.0012$^{+0.0001}_{-0.0001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 50499 b & 53175558 & 0.0012$^{+0.0003}_{-0.0002}$ & 0.000026$^{+0.000006}_{-0.000005}$ & 6,7 & 3,3 & \nodata & \nodata\\
HD 220773 b & 315415155 & 0.0012$^{+0.0003}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 160691 c & 406317882 & 0.0012$^{+0.0002}_{-0.0001}$ & 0.0000076$^{+0.000001}_{-0.0000009}$ & 12 & 1 & \nodata & \nodata\\
HD 154345 b & 313709116 & 0.00112$^{+0.00007}_{-0.00007}$ & 0.000018$^{+0.000001}_{-0.000001}$ & \nodata & \nodata & 11,12 & 3,3\\
GJ 179 b & 450102450 & 0.0011$^{+0.0001}_{-0.0001}$ & 0.000013$^{+0.000002}_{-0.000001}$ & 5 & 1 & \nodata & \nodata\\
HD 34445 g & 162494287 & 0.0011$^{+0.0002}_{-0.0002}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 150706 b & 380086262 & 0.0011$^{+0.002}_{-0.0005}$ & 0.00002$^{+0.00003}_{-0.00001}$ & \nodata & \nodata & 5,6,7,8 & 4,3,3,4\\
HD 134987 c & 246937460 & 0.0011$^{+0.0001}_{-0.0001}$ & 0.0000058$^{+0.0000008}_{-0.0000006}$ & 11 & 1 & \nodata & \nodata\\
HD 113538 c & 75377076 & 0.00105$^{+0.00007}_{-0.00006}$ & 0.000016$^{+0.000001}_{-0.000001}$ & 11 & 2 & \nodata & \nodata\\
HD 125612 d & 12906712 & 0.001$^{+0.0002}_{-0.0001}$ & \nodata & \nodata & \nodata & \nodata & \nodata\\
HD 74156 c & 379949822 & 0.00104$^{+0.00004}_{-0.00003}$ & 0.0000113$^{+0.0000004}_{-0.0000004}$ & 7 & 1 & \nodata & \nodata\\
WASP-8 c & 459558974 & 0.001$^{+0.0001}_{-0.0001}$ & 0.0000063$^{+0.0000009}_{-0.0000007}$ & 2 & 2 & \nodata & \nodata\\
HD 4203 c & 258444495 & 0.001$^{+0.0004}_{-0.0002}$ & 0.000004$^{+0.000002}_{-0.000001}$ & \nodata & \nodata & 3 & 1\\
HAT-P-17 c & 454082369 & 0.001$^{+0.001}_{-0.0004}$ & 0.000005$^{+0.000007}_{-0.000002}$ & \nodata & \nodata & 2 & 2\\
HD 142 c & 389757979 & 0.00093$^{+0.0001}_{-0.00009}$ & 0.0000042$^{+0.0000004}_{-0.0000004}$ & 2 & 2 & \nodata & \nodata\\
HD 95872 b & 52198580 & 0.00092$^{+0.00007}_{-0.00006}$ & 0.0000057$^{+0.0000004}_{-0.0000004}$ & 9 & 1 & \nodata & \nodata\\
55 Cnc d & 422478973 & 0.0009$^{+0.00002}_{-0.00002}$ & 0.0000051$^{+0.0000001}_{-0.0000001}$ & \nodata & \nodata & 7 & 1\\
HD 187123 c & 58559140 & 0.0009$^{+0.0001}_{-0.0001}$ & 0.0000062$^{+0.0000009}_{-0.0000007}$ & \nodata & \nodata & 1 & 3\\
GJ 832 b & 266593143 & 0.0009$^{+0.0004}_{-0.0004}$ & 0.000006$^{+0.000003}_{-0.000003}$ & 1 & 2 & \nodata & \nodata\\
HD 27894 d & 13105061 & 0.00086$^{+0.00008}_{-0.00006}$ & 0.000041$^{+0.000004}_{-0.000003}$ & 1,2,3,4,5,8,9,11,12 & 4,4,3,3,4,4,4,4,4 & \nodata & \nodata\\
HIP 70849 b & 127382459 & 0.0007$^{+0.003}_{-0.0007}$ & 0.000001$^{+0.000005}_{-0.000001}$ & 11 & 2 & \nodata & \nodata\\
HD 98649 b & 5078530 & 0.0007$^{+0.0004}_{-0.0003}$ & 0.000004$^{+0.000002}_{-0.000002}$ & 9 & 1 & \nodata & \nodata\\
HD 30177 c & 92352621 & 0.0007$^{+0.0001}_{-0.0001}$ & 0.000015$^{+0.000003}_{-0.000002}$ & 2,3,4,5,6,8,9,10,12,13 & 4,4,3,4,4,4,4,4,4,4 & \nodata & \nodata\\
GJ 328 b & 36853511 & 0.00057$^{+0.00004}_{-0.00003}$ & 0.0000038$^{+0.0000002}_{-0.0000002}$ & 8 & 1 & \nodata & \nodata\\
GJ 676 A c & 188580272 & 0.00057$^{+0.00005}_{-0.00005}$ & 0.0000021$^{+0.0000002}_{-0.0000002}$ & 12 & 1 & \nodata & \nodata\\
47 UMa d & 21535479 & 0.0006$^{+0.0003}_{-0.0003}$ & 0.0000011$^{+0.0000006}_{-0.0000005}$ & \nodata & \nodata & 8 & 2\\
HIP 5158 c & 268634769 & 0.0006$^{+0.0002}_{-0.0001}$ & 0.0000017$^{+0.0000006}_{-0.0000004}$ & 3 & 1 & \nodata & \nodata
